Inter-Level Cooperation in Hierarchical Reinforcement Learning

Hierarchies of temporally decoupled policies present a promising approach for enabling structured exploration in complex long-term planning problems. To fully achieve this approach an end-to-end training paradigm is needed. However, training these multi-level policies has had limited success due to challenges arising from interactions between the goal-assigning and goal-achieving levels within a hierarchy. In this article, we consider the policy optimization process as a multi-agent process. This allows us to draw on connections between communication and cooperation in multi-agent RL, and demonstrate the benefits of increased cooperation between sub-policies on the training performance of the overall policy. We introduce a simple yet effective technique for inducing inter-level cooperation by modifying the objective function and subsequent gradients of higher-level policies. Experimental results on a wide variety of simulated robotics and traffic control tasks demonstrate that inducing cooperation results in stronger performing policies and increased sample efficiency on a set of difficult long time horizon tasks. We also find that goal-conditioned policies trained using our method display better transfer to new tasks, highlighting the benefits of our method in learning task-agnostic lower-level behaviors. Videos and code are available at: https://sites.google.com/berkeley.edu/cooperative-hrl.

==> abstract.tex <==
\begin{abstract}
Hierarchies of temporally decoupled policies present a promising approach for enabling structured exploration in complex long term planning problems. To fully achieve this approach an end-to-end training paradigm is needed. However, training these multi-level policies has had limited success due to challenges arising from interactions between the goal-assigning and goal-achieving levels within a hierarchy. Drawing connections between these limitations and communication and cooperation in multi-agent RL, this paper demonstrates the benefits of increased cooperation between sub-policies on the training performance of the overall policy. We introduce a simple yet effective technique for inducing inter-level cooperation by modifying the objective function and subsequent gradients of higher-level policies. Experimental results on a wide variety of simulated robotics and traffic control tasks demonstrate that inducing cooperation results in stronger performing policies and increased sample efficiency on a set of difficult long time horizon tasks.
% Videos and code are available at: \url{https://sites.google.com/berkeley.edu/cooperative-hrl}.
\end{abstract}


==> background.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}
    \newcommand \boxwidth {0.65}
    \newcommand \boxoffset {0.5}
    \newcommand \envwidth {7.75}
    \newcommand \envheight {0.65}
    \newcommand \layerskip {1.4}

    % environment box
    \fill [orange!30!white] (0,0) rectangle (\envwidth, \envheight);
    \draw [brown] (0,0) -- (\envwidth,0);
    \draw [brown] (0, \envheight) -- (\envwidth, \envheight);
    \draw (\envwidth/2, \envheight/2) node {\small Environment};

    % Manager boxes
    \filldraw [black!40!white, draw=black!90!white] 
    (2*\boxoffset, 3.5*\envheight) rectangle 
    (2*\boxoffset + \boxwidth, 3.5*\envheight + \boxwidth);
    \draw
    (2.0*\boxoffset + 0.5*\boxwidth, 3.5*\envheight + 0.5*\boxwidth) node {\small $\pi_m$};

    % Worker boxes
    \filldraw [black!20!white, draw=black!80!white] 
    (4.5*\boxoffset, 2*\envheight) rectangle 
    (4.5*\boxoffset + \boxwidth, 2*\envheight + \boxwidth);
    \draw
    (4.5*\boxoffset + 0.5*\boxwidth, 2*\envheight + 0.5*\boxwidth) node {\small $\pi_w$};

    \filldraw [black!20!white, draw=black!80!white] 
    (6.0*\boxoffset + 1.0*\boxwidth, 2*\envheight) rectangle 
    (6.0*\boxoffset + 2.0*\boxwidth, 2*\envheight + \boxwidth);
    \draw
    (6.0*\boxoffset + 1.5*\boxwidth, 2*\envheight + 0.5*\boxwidth) node {\small $\pi_w$};

    \filldraw [black!20!white, draw=black!80!white] 
    (9.0*\boxoffset + 2.0*\boxwidth, 2*\envheight) rectangle 
    (9.0*\boxoffset + 3.0*\boxwidth, 2*\envheight + \boxwidth);
    \draw
    (9.0*\boxoffset + 2.5*\boxwidth, 2*\envheight + 0.5*\boxwidth) node {\small $\pi_w$};

    % connections

    \draw [->] 
    (1.25 * \boxoffset, \envheight) -- (1.25 * \boxoffset, 4 * \envheight) -- (2*\boxoffset, 4 * \envheight);
    \draw [->] 
    (1.25 * \boxoffset, 2.5*\envheight) -- (4.5*\boxoffset, 2.5*\envheight);
    \draw 
    (1.25 * \boxoffset + 0.25, \envheight + 0.2) node {\small $s_t$}; 

    \draw [->] 
    (2*\boxoffset + \boxwidth, 4*\envheight) -- 
    (4.5*\boxoffset + 0.5*\boxwidth, 4*\envheight) -- 
    (4.5*\boxoffset + 0.5*\boxwidth, 3*\envheight);
    \draw [->] 
    (4.5*\boxoffset + 0.5*\boxwidth, 4*\envheight) -- 
    (4.5*\boxoffset + 2.5*\boxwidth, 4*\envheight) -- 
    (4.5*\boxoffset + 2.5*\boxwidth, 3*\envheight);
    \draw 
    (4.5*\boxoffset + 2.5*\boxwidth, 4*\envheight) -- 
    (5.5*\boxoffset + 2.5*\boxwidth, 4*\envheight); 
    \draw 
    (7.5*\boxoffset + 2.0*\boxwidth, 4.0*\envheight) node {$\cdots$}; 
    \draw [->]
    (8.5*\boxoffset + 2.0*\boxwidth, 4*\envheight) -- 
    (9.0*\boxoffset + 2.5*\boxwidth, 4*\envheight) --
    (9.0*\boxoffset + 2.5*\boxwidth, 3*\envheight); 
    \draw 
    (2*\boxoffset + \boxwidth + 0.3, 4 * \envheight + 0.2) node {\small $g_t$}; 


    \draw [->] 
    (4.5*\boxoffset + \boxwidth, 2.5*\envheight) --
    (5.0*\boxoffset + \boxwidth, 2.5*\envheight) --
    (5.0*\boxoffset + \boxwidth, 1.0*\envheight);
    \draw
    (5.0*\boxoffset + \boxwidth - 0.25, \envheight + 0.2) node {\small $a_t$}; 

    \draw [->] 
    (5.5*\boxoffset + \boxwidth, 1.0*\envheight) --
    (5.5*\boxoffset + \boxwidth, 2.5*\envheight) --
    (6.0*\boxoffset + \boxwidth, 2.5*\envheight);
    \draw
    (5.5*\boxoffset + \boxwidth + 0.4, \envheight + 0.2) node {\small $s_{t+1}$}; 

    \draw [->] 
    (6.0*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
    (6.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
    (6.5*\boxoffset + 2.0*\boxwidth, 1.0*\envheight);
    \draw
    (6.5*\boxoffset + 2.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $a_{t+1}$}; 

    \draw (7.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) node {$\cdots$}; 

    \draw [->] 
    (8.5*\boxoffset + 2.0*\boxwidth, 1.0*\envheight) --
    (8.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
    (9.0*\boxoffset + 2.0*\boxwidth, 2.5*\envheight);
    \draw
    (8.5*\boxoffset + 2.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $s_{t+i}$}; 

    \draw [->] 
    (9.0*\boxoffset + 3.0*\boxwidth, 2.5*\envheight) --
    (9.5*\boxoffset + 3.0*\boxwidth, 2.5*\envheight) --
    (9.5*\boxoffset + 3.0*\boxwidth, 1.0*\envheight);
    \draw
    (9.5*\boxoffset + 3.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $a_{t+i}$};

    % ============================================================ %
    % ============================================================ %
    %               Draw the top (highway) network.                %
    % ============================================================ %
    % ============================================================ %

    \newcommand \lanewidth {0.5}
    \newcommand \lanepos {5.5*\envheight}

    % draw the lane
    \filldraw [black!20!white] 
    (0, \lanepos) rectangle (\textwidth, \lanepos + \lanewidth);
    \draw (0, \lanepos) -- (\textwidth, \lanepos);
    \draw (0, \lanepos + \lanewidth) -- (\textwidth, \lanepos + \lanewidth);

    % draw the individual vehicles

    \node[inner sep=0pt] at 
    (1.5, \lanepos + 0.5 * \lanewidth)
    {\includegraphics[origin=c,height=0.5cm]{figures/car.png}};

    \node[inner sep=0pt] at 
    (4.0, \lanepos + 0.5 * \lanewidth)
    {\includegraphics[origin=c,height=0.5cm]{figures/car.png}};

    \node[inner sep=0pt] at 
    (6.0, \lanepos + 0.5 * \lanewidth)
    {\includegraphics[origin=c,height=0.5cm]{figures/car.png}};

    \node[inner sep=0pt] at 
    (8.0, \lanepos + 0.5 * \lanewidth)
    {\includegraphics[origin=c,height=0.5cm]{figures/smartcar.png}};

    \node[inner sep=0pt] at 
    (10.5, \lanepos + 0.5 * \lanewidth)
    {\includegraphics[origin=c,height=0.5cm]{figures/car.png}};

    \node[inner sep=0pt] at 
    (14.5, \lanepos + 0.5 * \lanewidth)
    {\includegraphics[origin=c,height=0.5cm]{figures/car.png}};
    
    % draw the speedometer and goal
    
    \newcommand \speedometerCenterX {10.25}
    \newcommand \speedometerCenterY {1.25}
    \newcommand \speedometerRadius  {1.25}

    \newcommand \cosOne        {1}                    % cos(0)
    \newcommand \sinOne        {0}                    % sin(0)
    \newcommand \cosTwo        {0.9876883405951378}   % cos(9)
    \newcommand \sinTwo        {0.1564344650402308}   % sin(9)
    \newcommand \cosThree      {0.9510565162951535}   % cos(18)
    \newcommand \sinThree      {0.3090169943749474}   % sin(18)
    \newcommand \cosFour       {0.8910065241883679}   % cos(27)
    \newcommand \sinFour       {0.4539904997395467}   % sin(27)
    \newcommand \cosFive       {0.8090169943749475}   % cos(36)
    \newcommand \sinFive       {0.5877852522924731}   % sin(36)
    \newcommand \cosSix        {0.7071067811865476}   % cos(45)
    \newcommand \sinSix        {0.7071067811865476}   % sin(45)
    \newcommand \cosSeven      {0.5877852522924731}   % cos(54)
    \newcommand \sinSeven      {0.8090169943749475}   % sin(54)
    \newcommand \cosEight      {0.4539904997395467}   % cos(63)
    \newcommand \sinEight      {0.8910065241883679}   % sin(63)
    \newcommand \cosNine       {0.3090169943749474}   % cos(72)
    \newcommand \sinNine       {0.9510565162951535}   % sin(72)
    \newcommand \cosTen        {0.1564344650402308}   % cos(81)
    \newcommand \sinTen        {0.9876883405951378}   % sin(81)
    \newcommand \cosEleven     {0}                    % cos(90)
    \newcommand \sinEleven     {1}                    % sin(90)
    \newcommand \cosTwelve     {-0.1564344650402308}  % cos(99)
    \newcommand \sinTwelve     {0.9876883405951378}   % sin(99)
    \newcommand \cosThirteen   {-0.3090169943749474}  % cos(108)
    \newcommand \sinThirteen   {0.9510565162951535}   % sin(108)
    \newcommand \cosFourteen   {-0.4539904997395467}  % cos(117)
    \newcommand \sinFourteen   {0.8910065241883679}   % sin(117)
    \newcommand \cosFifteen    {-0.5877852522924731}  % cos(126)
    \newcommand \sinFifteen    {0.8090169943749475}   % sin(126)
    \newcommand \cosSixteen    {-0.7071067811865476}  % cos(135)
    \newcommand \sinSixteen    {0.7071067811865476}   % sin(135)
    \newcommand \cosSeventeen  {-0.8090169943749475}  % cos(144)
    \newcommand \sinSeventeen  {0.5877852522924731}   % sin(144)
    \newcommand \cosEighteen   {-0.8910065241883679}  % cos(153)
    \newcommand \sinEighteen   {0.4539904997395467}   % sin(153)
    \newcommand \cosNineteen   {-0.9876883405951378}  % cos(162)
    \newcommand \sinNineteen   {0.1564344650402308}   % sin(162)
    \newcommand \cosTwenty     {-0.9510565162951535}  % cos(171)
    \newcommand \sinTwenty     {0.3090169943749474}   % sin(171)
    \newcommand \cosTwentyOne  {-1}                   % cos(180)
    \newcommand \sinTwentyOne  {0}                    % sin(180)

    \newcommand \cosSpeed      {0.20791169081775945}
    \newcommand \sinSpeed      {0.9781476007338056}
    \newcommand \cosGoal       {0.927183854566787}
    \newcommand \sinGoal       {0.374606593415912}

    % point to speedometer
    \draw 
    (8.00, \lanepos - 0.50 * \lanewidth) --
    (9.00, \lanepos - 2.75 * \lanewidth);

    % draw speedometer
    \draw [line width=0.35mm]
    (\speedometerCenterX + 0.75 * \speedometerRadius * \cosOne,
     \speedometerCenterY + 0.75 * \speedometerRadius * \sinOne) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosOne,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinOne);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosTwo,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinTwo) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosTwo,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinTwo);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosThree,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinThree) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosThree,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinThree);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosFour,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinFour) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosFour,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinFour);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosFive,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinFive) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosFive,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinFive);
    \draw [line width=0.35mm]
    (\speedometerCenterX + 0.75 * \speedometerRadius * \cosSix,
     \speedometerCenterY + 0.75 * \speedometerRadius * \sinSix) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosSix,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinSix);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosSeven,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinSeven) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosSeven,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinSeven);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosEight,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinEight) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosEight,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinEight);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosNine,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinNine) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosNine,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinNine);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosTen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinTen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosTen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinTen);
    \draw [line width=0.35mm]
    (\speedometerCenterX + 0.75 * \speedometerRadius * \cosEleven,
     \speedometerCenterY + 0.75 * \speedometerRadius * \sinEleven) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosEleven,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinEleven);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosTwelve,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinTwelve) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosTwelve,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinTwelve);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosThirteen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinThirteen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosThirteen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinThirteen);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosFourteen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinFourteen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosFourteen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinFourteen);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosFifteen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinFifteen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosFifteen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinFifteen);
    \draw [line width=0.35mm]
    (\speedometerCenterX + 0.75 * \speedometerRadius * \cosSixteen,
     \speedometerCenterY + 0.75 * \speedometerRadius * \sinSixteen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosSixteen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinSixteen);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosSeventeen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinSeventeen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosSeventeen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinSeventeen);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosEighteen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinEighteen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosEighteen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinEighteen);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosNineteen,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinNineteen) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosNineteen,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinNineteen);
    \draw [line width=0.25mm]
    (\speedometerCenterX + 0.90 * \speedometerRadius * \cosTwenty,
     \speedometerCenterY + 0.90 * \speedometerRadius * \sinTwenty) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosTwenty,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinTwenty);
    \draw [line width=0.35mm]
    (\speedometerCenterX + 0.75 * \speedometerRadius * \cosTwentyOne,
     \speedometerCenterY + 0.75 * \speedometerRadius * \sinTwentyOne) --
    (\speedometerCenterX + 1.00 * \speedometerRadius * \cosTwentyOne,
     \speedometerCenterY + 1.00 * \speedometerRadius * \sinTwentyOne);

    % draw goal
    \draw [line width=0.5mm, color=blue]
    (\speedometerCenterX + 0.0 * \speedometerRadius * \cosGoal,
     \speedometerCenterY + 0.0 * \speedometerRadius * \sinGoal) --
    (\speedometerCenterX + 1.0 * \speedometerRadius * \cosGoal,
     \speedometerCenterY + 1.0 * \speedometerRadius * \sinGoal);
    \draw 
    (\speedometerCenterX + 1.15 * \speedometerRadius * \cosGoal + 0.3,
     \speedometerCenterY + 1.15 * \speedometerRadius * \sinGoal) node {\small \textcolor{blue}{goal}}; 

    % draw current speed
    \draw [line width=0.5mm, color=red]
    (\speedometerCenterX + 0.0 * \speedometerRadius * \cosSpeed,
     \speedometerCenterY + 0.0 * \speedometerRadius * \sinSpeed) --
    (\speedometerCenterX + 1.0 * \speedometerRadius * \cosSpeed,
     \speedometerCenterY + 1.0 * \speedometerRadius * \sinSpeed);
    \draw 
    (\speedometerCenterX + 1.15 * \speedometerRadius * \cosSpeed + 1,
     \speedometerCenterY + 1.15 * \speedometerRadius * \sinSpeed) node {\small \textcolor{red}{current speed}}; 

    % draw the center point
    \filldraw (\speedometerCenterX,\speedometerCenterY) circle (0.05 * \speedometerRadius);

    % ============================================================ %
    % ============================================================ %
    %              Draw the right (Ant) environment.               %
    % ============================================================ %
    % ============================================================ %
    
    \hspace*{0.8\textwidth}\includegraphics[width=0.2\textwidth]{figures/ant-goal.png}

\end{tikzpicture}\\[-8pt]
\caption{An illustration of the studied hierarchical model. \textbf{Left:} A manager network $\pi_m$ issues commands (or goals) $g_t$ over $k$ consecutive time steps to a worker $\pi_w$. The worker then performs environment actions $a_t$ to accomplish these goals. \textbf{Top/right:} The commands issued by the manager denote desired states for the worker to traverse. For the AV control tasks, we define the goal as the desired speeds for each AV. Moreover, for agent navigation tasks, the goals are defined as the desired position and joint angles of the agent.}
\label{fig:hrl-model}
\end{figure*}

\section{Background} \label{sec:background}

% \subsection{Reinforcement learning and MDPs} 
% \label{sec:mdps-rl}

RL problems are generally studied as a \emph{Markov decision problem} (MDP) \citep{bellman1957markovian}, defined by the tuple: $(\mathcal{S}, \mathcal{A}, \mathcal{P}, r, \rho_0, \gamma, T)$, where $\mathcal{S} \subseteq \mathbb{R}^n$ is an $n$-dimensional state space, $\mathcal{A} \subseteq \mathbb{R}^m$ an $m$-dimensional action space, $\mathcal{P} : \mathcal{S} \times \mathcal{A} \times \mathcal{S} \to \mathbb{R}_+$ a transition probability function, $r : \mathcal{S} \to \mathbb{R}$ a reward function, $\rho_0 : \mathcal{S} \to \mathbb{R}_+$ an initial state distribution, $\gamma \in (0,1]$ a discount factor, and $T$ a time horizon. 

In a MDP, an \textit{agent} is in a state $s_t \in \mathcal{S}$ in the environment and interacts with this environment by performing actions $a_t \in \mathcal{A}$. The agent's actions are defined by a policy $\pi_\theta : \mathcal{S} \times \mathcal{A} \to \mathbb{R}_+$ parametrized by $\theta$. The objective of the agent is to learn an optimal policy: $\theta^* := \text{argmax}_\theta J(\pi_\theta)$, where $J(\pi_\theta) = \mathbb{E}_{p\sim \pi_\theta} \left[ \sum_{i=0}^T \gamma^i r_i\right]$ is the expected discounted return.

% \subsection{Actor-critic algorithms} \label{sec:actor-critic}
% Several algorithms have been proposed for computing an optimal policy under the aforementioned formulation. With gradient based methods, the policy is updated by taking
% the gradient of the expected return $\nabla_\theta J(\theta)$~\cite{sutton2000policy}. In a specific class of actor-critic methods particularly well suited for continuous action spaces, the gradient of a continuous policy, or actor, is computed through the deterministic policy gradient algorithm~\cite{silver2014deterministic}:
% \begin{equation}
% 	\nabla_\theta J (\theta) = \mathbb{E}_{s\sim p_\pi} \left[ \nabla_a Q_\phi (s,a)|_{a=\pi(s)}\nabla_\theta \pi_\theta(s) \right]
% \end{equation}
% where $Q_\phi(s,a) = \mathbb{E}_{s_i\sim p_\pi, a_i \sim \pi} [\sum_{i=t}^T \gamma^{i-t} r_i|s,a]$ is the expected return from a starting state $s$ given an action $a$. This value function is estimated by an additional function approximator, known as a critic, which is learned using temporal difference learning \cite{sutton1988learning,watkins1992q}, an update rule based on the Bellman equation~\cite{bellman1957markovian}:
% \begin{equation} \label{eq:td-learning}
%     \varepsilon (s_t, a_t, s_{t+1}) = \left[ Q_\phi(s_t,a_t) - y \right] ^2
% \end{equation}
% where:
% \begin{equation}
%      y = r_t + \gamma Q_{\bar{\phi}} (s_{t+1}, \pi_\theta(s_{t+1}))
% \end{equation}
% and $Q_{\bar{\phi}}$ is a target Q function whose parameters are periodically updated with the most recent $\phi$. This target term is meant to help stabilize learning~\cite{mnih2015human}.

\subsection{Hierarchical reinforcement learning} \label{sec:background-hrl}
In HRL, the policy is decomposed into a high-level policy that optimizes the original task reward, and a low-level policy that is conditioned on latent goals from the high-level and executes actions within the environment. The high-level controller is decoupled from the true MDP by operating at a lower temporal resolution and passing goals~\citep{dayan1993feudal} or options~\citep{sutton1999between} to the lower-level. This can reduce the credit assignment problem from the perspective of the high-level controller, and allows the low-level policy to produce action primitives that support short time horizon tasks as well~\citep{sutton1999between}.

Several HRL frameworks have been proposed to facilitate and/or encourage the decomposition of decision-making and execution during training~\citep{dayan1993feudal, sutton1999between, parr1998reinforcement, dietterich2000hierarchical}. In this paper, we consider a two-level goal-conditioned arrangement~\cite{vezhnevets2017feudal, nachum2018data, nasiriany2019planning} (see Figure~\ref{fig:hrl-model}). This network consists of a high-level, or manager, policy $\pi_m$ that computes and outputs goals $g_t \sim \pi_m(s_t)$ every $k$ time steps, and a low-level, or worker, policy $\pi_w$ that takes as inputs the current state and the assigned goals and is encouraged to perform actions $a_t \sim \pi_w(s_t, g_t)$ that satisfy these goals via an intrinsic reward function $r_w(s_t, g_t, s_{t+1})$ (see Appendix~\ref{sec:intrinsic-reward}).

\subsection{Hierarchical policy optimization} \label{sec:no-cooperation}

Goal-conditioned HRL considers a concurrent training procedure for the manager and worker policies. In this setting, the manager receives a reward based on the original environmental reward function: $r_m(s_t)$. The objective function from the perspective of the manager is then:\\[-3pt]
\begin{equation} \label{eq:manager-objective}
\resizebox{!}{12pt}{$
    J_m = \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^{T/k} \left[ \gamma^t r_m(s_t) \right] \right]
$}
\end{equation}
Conversely, the worker policy is motivated to follow the goals set by the manager via an intrinsic reward $r_w (s_t, g_t, s_{t+1})$ separate from the external reward. The objective function from the perspective of the worker is then:\\[-6pt]
\begin{equation} \label{eq:worker-objective}
\resizebox{!}{12pt}{$
    J_w = \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^k \gamma^t r_w(s_t, g_t,\pi_w(s_t,g_t)) \right]
$}
\end{equation}
% The update procedures for each policy are depicted in Fig.~\ref{fig:hrl-connected} (left). 
Notably, no gradients are shared between the manager and worker policies. 
% \todo{Removed content here to simplify the text.}
As discussed in Section~\ref{sec:introduction} and depicted in Figure~\ref{fig:goaldists}, the absence of such feedback often results in the formation of non-cooperative goal-assignment behaviors that further complicate the learning process. % The validity of this argument is explored in the following sections.


==> conclusion.tex <==
\section{Conclusions and future work} \label{sec:conclusions}

In this work, we propose connections between multi-agent and hierarchical reinforcement learning that motivates our novel method of inducing cooperation in hierarchies. We provide a derivation of the gradient of a manager policy with respect to its workers for an actor-critic formulation as well as introducing a $\lambda$ weighting term for this gradient which controls the level of cooperation. We find that using \methodName results in consistently better-performing policies, that have lower empirical non-stationarity than prior work, particularly for more difficult tasks.

For future work, we would like to apply this method to discrete action environments and additional hierarchical models such as the options framework. Potential future work also includes extending the cooperative HRL formulation to multi-level hierarchies, in which the multi-agent nature of hierarchical training is likely to be increasingly detrimental to training stability.

% We limit our derivation of the cooperative gradient to deterministic policy gradients as it a commonly studied RL algorithm in recent studies on HRL~\citep{levy2017hierarchical,nachum2018data,nachum2018near}, and as a result allows us to fairly compare the use of cooperative gradients to existing state-of-the-art methods. The derivation of this gradient to direct policy gradient~\citep{williams1992simple} and soft actor-critic~\citep{haarnoja2018soft} methods is a topic of future work.

% \section*{Acknowledgements}

% This work is supported by an AWS Machine Learning Research Award. This is also material is based upon work supported by the U.S. Department of Energy’s Office of Energy Efficiency and Renewable Energy (EERE) award number CID DE-EE0008872. The views expressed herein do not necessarily represent the views of the U.S. Department of Energy or the United States Government.


==> experiments.tex <==

\begin{figure*}
\begin{subfigure}[b]{\textwidth}
\centering
\begin{tikzpicture}
    \newcommand \boxwidth {1.0}
    \newcommand \boxheight {\textwidth}
    \newcommand \boxoffset {0}

    % for y shift
    \draw (0, -0.25) node {};

    % \draw
    % (\boxoffset,              \boxoffset) -- 
    % (\boxheight + \boxoffset, \boxoffset) -- 
    % (\boxheight + \boxoffset, \boxwidth + \boxoffset) -- 
    % (\boxoffset,              \boxwidth + \boxoffset) -- 
    % (\boxoffset,              \boxoffset);

    \draw [color=color1]
    (0.25, \boxwidth + \boxoffset - 0.5) -- 
    (1.00, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west] 
    (1.05, \boxwidth + \boxoffset - 0.5) node {\scriptsize TD3};

    \draw [color=color2]
    (2.25, \boxwidth + \boxoffset - 0.5) -- 
    (3.00, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west] 
    (3.05, \boxwidth + \boxoffset - 0.5) node {\scriptsize HRL};

    \draw [color=color3] 
    (4.25, \boxwidth + \boxoffset - 0.5) -- 
    (5.00, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west]
    (5.05, \boxwidth + \boxoffset - 0.5) node {\scriptsize HIRO};

    \draw [color=color4] 
    (6.25, \boxwidth + \boxoffset - 0.5) -- 
    (7.00, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west]
    (7.05, \boxwidth + \boxoffset - 0.5) node {\scriptsize HAC};

    \draw [color=color5] 
    (8.25, \boxwidth + \boxoffset - 0.5) -- 
    (9.00, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west]
    (9.05, \boxwidth + \boxoffset - 0.5) node {\scriptsize \methodName (fixed)};

    \draw [color=color6] 
    (11.25, \boxwidth + \boxoffset - 0.5) -- 
    (12.00, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west]
    (12.05, \boxwidth + \boxoffset - 0.5) node {\scriptsize \methodName (dynamic)};
\end{tikzpicture}
\end{subfigure} \\ \vspace{-0.4cm}
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/ring-v0-rewards.pdf}
    \caption{\footnotesize \ringroad}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/highway-v2-rewards.pdf}
    \caption{\footnotesize \highwaysingle}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/BipedalSoccer-results.pdf}
    \caption{\footnotesize \bipedalsoccer}
    \label{fig:biped-results}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.205\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather-rewards.pdf}
    \caption{\footnotesize \antgather}
\end{subfigure} \\ \vspace{0.2cm}
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntFourRooms-rewards.pdf}
    \caption{\footnotesize \antfourrooms}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntMaze-0-rewards.pdf}
    \caption{\footnotesize \antmaze [16,0]}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntMaze-1-rewards.pdf}
    \caption{\footnotesize \antmaze [16,16]}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntMaze-2-rewards.pdf}
    \caption{\footnotesize \antmaze [0,16]}
\end{subfigure}\\[-8pt]
\caption{Training performance of the different algorithms on various environments.
% \todoGlen{Need all figures to have results from all algorithms}
}
\label{fig:learning-curves}
\end{figure*}

\section{Experiments}
\label{sec:experiments}

%%GB.11.03: This entire section needs to be rewritten. The environments and other algorithms should not take up an entire page. This is great work and we need that space to outline the best parts of the results much better. MOST importantly these experiments need some organization. What are the experimental questions we want to ask? (1) Will CHER work? what kind of results does it give, (2) Is CHER more sample efficient than other methods (including other HRL methods). (3) How much for the adaptive \lambda help? (4) More ablations to understand the most important parts of the method. What is also missed in this paper in general is some understanding that these are difficult tasks, for example TD3 can not solve half of these. This should also be highlighted in the experiments again.

In this section, we detail the experimental setup and training procedure and present the performance of our method results of various continuous control tasks. Through these experiments, we aim to determine two things: \\[-20pt]
\begin{enumerate}[leftmargin=*,noitemsep]
    \item How does cooperation in HRL improve the behavior of goal-assignment strategies and the performance of the resulting policy?
    \item How important is it to control the varying degree of cooperation between learned higher and lower level behaviors?\\[-20pt]
\end{enumerate}
% \todo{In the future if the experiments on this work out, we can add: Does the use of communication results in a more structured goal condition lower level policy that transfers better to other tasks?}


% The experimental evaluation should be organized like this:

% 1. Does adding cooperation to the hierarchical reinforcement learning problem enable more efficient learning for difficult long horizon planning problems.
% 2. how does the degree of cooperation between the policy levels influence the learning efficiency?
% 3. How does the use of communication shape the exploration behavior in terms of goal assignments for the high-level policies and does this help the exploration and training problem.
% 4. Does the use of communication results in a more structured goal condition lower level policy that transfers better to other tasks?

All results within this section are reported over $10$ random seeds. Details on the choice of hyperparameters are provided in Appendix~\ref{sec:hyperparams}.

\subsection{Environments}

We explore the use of hierarchical reinforcement learning on a variety of difficult long time horizon tasks, see Figure~\ref{fig:envs}. These environments vary from agent navigation tasks (Figures~\ref{fig:antgather-env}~to~\ref{fig:biped-sim}), in which a robotic agent tries to achieve certain long-term goals, to two mixed-autonomy traffic control tasks (Figures~\ref{fig:ring-env}~to~\ref{fig:highwaysingle-env}), in which a subset of vehicles (seen in red) are treated as automated vehicles and attempt to reduce oscillations in vehicle speeds known as stop-and-go traffic. Further details are available in Appendix~\ref{sec:environments}.

The environments presented here pose a difficulty to standard RL methods for a variety of reasons. We broadly group the most significant of these challenges into two categories: temporal reasoning and delayed feedback.

% \noindent \textbf{Multi-level reasoning} \ \ \
\textbf{Temporal reasoning} \ \
In the agent navigation tasks, the agent must learn to perform multiple tasks at varying levels of granularity. At the level of individual timesteps, the agent must learn to navigate its surroundings, moving up, down, left, or right without falling or dying prematurely. More macroscopically, however, the agent must exploit these action primitives to achieve high-level goals that may be sparsely defined or require exploration across multiple timesteps. For even state-of-the-art RL algorithms, the absence of hierarchies in these settings result in poor performing policies in which the agent stands still or follows sub-optimal greedy behaviors.
% in which an agent stands still in very sparse settings such the \antgather environment, or follows greedy or non-optimal trajectories, such as moving diagonally in the \antfourrooms environment when trying to reach the space two rooms apart.

\textbf{Delayed feedback} \ \
In the mixed autonomy traffic tasks, meaningful events occur over large periods of time, as oscillations in vehicle speeds propagate slowly through a network. As a result, actions often have a delayed effect on metrics of improvement or success, making reasoning on whether a certain action improved the state of traffic a particularly difficult task. The delayed nature of this feedback prevents standard RL techniques from generating meaningful policies without relying on reward shaping techniques which produce undesirable behaviors such as creating large gaps between vehicles~\cite{wu2017flow}.

% In the mixed autonomy traffic tasks, actions by individual vehicles often have a delayed effect on metrics of improvement or success. Oscillations in vehicle speeds, which are a significant source of traffic congestion, propagate slowly through a network, at times requiring hundreds of steps to meaningfully affect the flow of vehicles, and as such the reward assigned to learning policies. This makes reasoning on whether a certain action contributed to or mitigated the formation of traffic oscillations a particularly difficult task. The delayed nature of this feedback prevents standard RL techniques from generating meaningful policies without relying on reward shaping techniques which produce undesirable behaviors such as creating large gaps between vehicles~\citep{wu2017flow}. We aim here to learn similar or better performing policies in the absence of reward shaping.


\begin{figure*}
\centering
% \begin{subfigure}[b]{0.2\textwidth}
%     \centering
% \end{subfigure}
% \hfill
\begin{subfigure}[b]{\textwidth}
\begin{tikzpicture}
    \newcommand \boxwidth {1.0}
    \newcommand \boxheight {\textwidth}
    \newcommand \boxoffset {0}

    % for y shift
    \draw (0, -0.15) node {};

    \filldraw [blue] (0.705 * \textwidth, \boxwidth + \boxoffset - 0.5) circle (0.125);
    \draw [anchor=west]
    (0.72 * \textwidth, \boxwidth + \boxoffset - 0.5) node {\scriptsize High-level goal};

    \draw [dashed] 
    (0.840 * \textwidth, \boxwidth + \boxoffset - 0.5) -- 
    (0.875 * \textwidth, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west]
    (0.88 * \textwidth, \boxwidth + \boxoffset - 0.5) node {\scriptsize Agent trajectory};
\end{tikzpicture}
\end{subfigure} \\ \vspace{-0.4cm}
\begin{subfigure}[b]{0.08\textwidth}
    \small{Standard\\ HRL} \\[10pt]
    
    \textcolor{white}{.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=0.48\linewidth]{figures/ring_hrl.png}
    \hfill
    \includegraphics[width=0.48\linewidth]{figures/ring_hrl.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/antgather_hrl.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\linewidth]{figures/antfourrooms_hrl.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/antmaze_hrl.pdf}
\end{subfigure}
\\[5pt]
\begin{subfigure}[b]{0.08\textwidth}
    \small{\methodName\\ (ours)} \\[25pt]
    
    \textcolor{white}{.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=0.48\linewidth]{figures/ring_cher.png}
    \hfill
    \includegraphics[width=0.48\linewidth]{figures/ring_cher.pdf}
    \caption{\ringroad}
    \label{fig:ring-traj}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/antgather_cher.pdf}
    \caption{Gather}
    \label{fig:antgather-traj}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\linewidth]{figures/antfourrooms_cher.pdf}
    \caption{Four Rooms}
    \label{fig:antfourrooms-traj}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/antmaze_cher.pdf}
    \caption{\footnotesize Maze}
    \label{fig:antmaze-traj}
\end{subfigure}\\[-8pt]
\caption{Illustration of the agent and goal trajectories for some of the environments studied here. The high-level goals learned via \methodName more closely match the agents' trajectories as they traverse the various environments. This results in improved dynamical behaviors by the agent in a majority of the tasks.}
\label{fig:goal-trajectories}
\end{figure*}

\subsection{Baseline algorithms}
% We begin by comparing the performance of \methodName against a variety of state-of-the-art hierarchical and non-hierarchical reinforcement learning algorithms. 
We test our proposed algorithm against the following baseline methods:\\[-15pt]
\begin{itemize}[leftmargin=*,noitemsep]
    \item \textit{TD3}: To validate the need for goal-conditioned hierarchies to solve our tasks, we compare all results against a fully connected network with otherwise similar network and training configurations.
    \item \textit{HRL}: This baseline consists of the naive formulation of the hierarchical reinforcement learning optimization scheme (see Section~\ref{sec:no-cooperation}). This algorithm is analogous to the \methodName algorithm with $\lambda$ set to $0$.
    \item \textit{HIRO}: Presented by~\citet{nachum2018data}, this method addresses the non-stationarity effects between the manager and worker policies by relabeling the manager's actions (or goals) to render the observed action sequence more likely to have occurred by the current instantiation of the worker policy. 
    % This is done by sampling a sequence of potential goals via a Gaussian centered at $s_{t+k}-s_t$ and choosing the candidate goal that maximizes the log-probability of the actions that were originally performed by the worker. 
    % This algorithm, at the time of writing, represents the state-of-the-art in goal-conditioned HRL. 
    The reproducibility of this algorithm is addressed in Appendix~\ref{sec:hiro-reproducibility}.
    \item \textit{HAC}: 
    % Similar to the HIRO algorithm, t
    The HAC algorithm~\citep{levy2017hierarchical} attempts to address non-stationarity in off-policy learning by relabeling sampled data via hindsight action and goal transitions
    % from an optimal lower-level policy 
    as well as subgoal testing transitions to prevent learning from a restricted set of subgoal states. Implementation details 
    % and modifications to this algorithm 
    are provided in Appendix~\ref{sec:hac-egocentric}.\\[-15pt]
\end{itemize}

% \subsection{Experimental setup}
% \label{sec:exp-setup}

% Experiments were conducted using TD3 as the underlying learning algorithm~\cite{fujimoto2018addressing}.
% , a variant of the DDPG~\cite{lillicrap2015continuous} algorithm for continuous control that utilizes dual value functions and delaying policy updates to reduce overestimation bias.

\subsection{Comparative analysis}

Figure~\ref{fig:learning-curves} depicts the training performance of each of the above algorithms on the studied tasks. We find that \methodName performs comparably or outperforms all other studied algorithms for the provided tasks. Interestingly, \methodName particularly outperforms other algorithms in highly stochastic and partially observable tasks. For the \antgather and traffic control tasks, in particular, the objective (be it the positions of apples and bombs or the density and driving behaviors within a traffic network) varies significantly at the start of a new rollout and is not fully observable to the agent from its local observation. As such, the improved performance by \methodName within these settings suggests that it is more robust than previous methods to learning policies that generalize to a wider set of problems as opposed to overfitting to a specific solution.

The improvements presented above emerge in part from more informative goal-assignment behaviors by the \methodName algorithm. Figure~\ref{fig:goal-trajectories} depicts these behaviors for a large number of tasks. We describe some of these behaviors and the subsequent performance of the policy below.

For the agent navigation tasks, the \methodName algorithm produces goals that more closely match the agent's trajectory, providing the agent with a more defined path to follow to achieve certain goals. This results in faster and more efficient learning for settings such as \antfourrooms, and in stronger overall policies for tasks such as \antgather. An interesting corollary that appears to emerge as a result of this cooperative approach is more stable movements and actuation commands by the worker policy. For settings in which the agent can fall prematurely, this appears in the form of fewer early terminations as a result of agents attempting to achieve difficult or highly random goals. The absence of frequent early terminations allows the policy to explore further into its environment during training; this is undoubtedly a benefit in settings where long-term reasoning is crucial.

% For the \ringroad environment for instance, while standard hierarchical methods produce unstable, 

In the \ringroad environment, we find standard HRL techniques fail to learn goal-assignment strategies that yield meaningful performative benefits. Instead, as seen in Figure~\ref{fig:ring-traj} (top), the manager overestimates its worker's ability to perform certain tasks and assign maximum desired speeds. This strategy prevents the policy from dissipating the continued propagation of vehicle oscillations in the network, as the worker policy is forced to assign large acceleration to match the desired speeds thereby contributing to the formation of stop-and-go traffic, seen as the red diagonal streaks in Figure \ref{fig:ring-traj}, top-left.
% 
% A similar phenomena is experienced in the \highwaysingle environment, with AV control strategies not providing meaningful improvements over uncontrolled, or human-driven, baselines (see Figure~\ref{fig:ts-no-control}).
% 
For these tasks, we find that inducing inter-level cooperation serves to alleviate the challenge of overestimating certain goals. In the \ringroad environment, for instance, \methodName succeeds in assigning meaningful desired speeds that encourage the worker policy to reduce the magnitude of accelerations assigned while near the free-flow, or optimal, speed of the network. This serves to eliminate the formation of stop-and-go traffic both from the perspective of the automated and human-driven vehicles, as seen in Figure \ref{fig:ring-traj}, bottom. We also note that when compared to previous studies of a similar task~\citep{wu2017flow}, our approach succeeds in finding a solution that does not rely on the generation of large or undesirable gaps between the AV and its leader. Similar results for the \highwaysingle environment are provided in Appendix~\ref{appendix:highway-results}.

% Similar improvements are witnessed within the \highwaysingle environment, as seen in Figure~\ref{fig:highwaysingle-results}. In this setting, multiple interacting AVs learn to develop spacing arrangements that prevent downstream congestion phenomena from fully propagating through the controllable region of traffic. This provides significant improves to the average speed of traffic within this controllable region.

% For both the tasks highlighted above, we find that only \methodName is successful in learning meaningful control strategies across all random seeds.


\begin{figure*}
\centering
\begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather-effects-worker-qvals.pdf}
    \caption{Worker expected returns}
    \label{fig:cg-delta-worker-qvals}
\end{subfigure}
\qquad
\begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather-effects-cg-delta.pdf}
    \caption{Evolution of dynamic $\lambda$}
    \label{fig:cg-delta-lambda}
\end{subfigure}
\qquad
\begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather-cg-delta.pdf}
    \caption{Effects of cooperation}
    \label{fig:cg-delta-rewards}
\end{subfigure}\\ \vspace{0.5cm}
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather/HRL/0.pdf}
    \caption{0\%} \label{fig:antgather-0p}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather/delta=-300/0.pdf}
    \caption{50\%} \label{fig:antgather-50p}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather/delta=-200/0.pdf}
    \caption{66.7\%} \label{fig:antgather-66.7p}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather/delta=-150/0.pdf}
    \caption{75\%} \label{fig:antgather-75p}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather/delta=-100/0.pdf}
    \caption{83.3\%} \label{fig:antgather-83.3p}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/AntGather/delta=-50/0.pdf}
    \caption{91.7\%} \label{fig:antgather-91.7p}
\end{subfigure}\\[-8pt]
\caption{Effect of varying degrees of cooperation for the \antgather environment. We plot the performance of the optimal policy and sample trajectories for various cooperation ratios as defined in Section~\ref{sec:cg-weight} (see the subcaptions for d-i). Increasing degrees of cooperation improve the agent's ability to assign desired goals that match the agent's trajectory, which subsequently improves the performance of the policy. Large degrees of cooperation, however, begin to disincentivize the agent from moving.}
\label{fig:effect-of-cg-weights}
\end{figure*}

% \subsubsection{Agent navigation environments}

% In the \antgather environment, this assist the agent as it attempts to avoid avoiding the bombs (in red), and both training and evaluation results in fewer early terminations as a result of attempting to achieve difficult goals. This results in policy receiving on average $4.10 \pm 0.18$ apples vs. bombs from the \methodName algorithm as opposed to $3.04 \pm 0.54$ via typical hierarchical techniques. Moreover, in the \antfourrooms environment, our method is capable of learning a policy after 1 million steps that navigates the agent both to the sides of the environment as well as to the diagonal room via one of the adjacent rooms. Within the same period of time the policy learned under the standard HRL objectification scheme continues pursue the more greedy as less optimal path, as seen in Figure~\ref{fig:antfourrooms-traj}. Finally, in the AntMaze environment, while \methodName does learn to perform optimally slightly earlier, we find no significant differences between the performance and \methodName and other algorithms. This is likely due to the fact that the goals assigned to the policy do no need to be particularly intricate for the agent to follow the desired trajectory, as seen in Figure \ref{fig:antmaze-traj}. Additional finding from vision-based variants of the \antmaze environment (see Appendix~\ref{sec:visual-antmaze}) suggest that utilizing cooperation can subvert the computational complexity of algorithms such as HIRO, thereby solving for optimal policies with a far smaller wall-clock time.

% We first perform a sample efficiency study designed to examine how effective \methodName is compared to related methods.
% Figure~\ref{fig:learning-curves} depicts the training performance of each algorithm for the various environments described in the Section~\ref{sec:environments}. In many cases, the use of cooperative higher-level objectives empirically provides significant improvements on the optimal performance of the policy within the environment. In the \antgather and \highwaysingle environments, while the \methodName policy originally progresses more slowly than standard HRL, it is ultimately capable of outperforming all other polices, producing a maximum return of $4.10 \pm 0.18$ and $4546 \pm 431$, respectively, across $10$ policies. This serves to far exceed the standard HRL algorithm's maximum return of $3.04 \pm 0.54$ and $3852 \pm 200$, respectively. The \methodName algorithm also exhibits more stable training in the \antgather environment, yielding a much smaller variance in performance between seeds.


% In the \ringroad and \highwaysingle environment in particular, \methodName enables the generation of meaningful traffic flow control behaviors by the automated vehicles (see Figure~\ref{fig:ts-control} for the \highwaysingle). This is in stark contrast to the non-hierarchical and standard HRL approaches, in which the learned control strategies do not result in significant improvements to the traveling speed of traffic, as seen in Figure~\ref{fig:avg-speed}. These results indicate that \methodName has (1) improved over current methods, and (2) expanded the space of control tasks that can be solved with HRL methods.
% \footnote{Additional results for the \ringroad environment can be found in Appendix~\ref{sec:ring-road-results}.}.

% Similar improvements can be seen in the \antmaze tasks in Figure~\ref{fig:learning-curves}(d-f). In this case, \methodName performs approximately equivalently to the HRL algorithm for simple goals, in this case moving to (16,0), i.e. simply moving forward. However, for the more difficult tasks \methodName converges several hundreds of thousands of steps prior to the standard HRL approach, and is comparable to the HIRO algorithm in terms of sample efficiency. Unlike HIRO, \methodName does not rely on relabeling techniques that are computationally expensive, and \methodName achieves greater evaluation performance than HIRO, at a lower wall-clock time. This is discussed in Appendix~\ref{sec:visual-antmaze}.

% We find similar results in the \bipedalsoccer task, shown in Figure~\ref{fig:biped-results}. For this task in particular the goal space is large making it difficult for HIRO to learn efficiently. Our method is able to outperform HIRO by completing the task in only half the number of environment steps. We also find that HAC was not able to solve the task and is not shown.

% The improvements in environmental returns in all tasks are equally coupled with a set of improvements in the intrinsic returns as seen in Figure~\ref{fig:effect-of-cg-weights}, thereby validating the of ability of the \methodName algorithm to improve cooperation between the two policies. %These results both indicate that \methodName has (1) improved over current methods and (2) expanded the space of control tasks that can be solved with HRL methods.

\subsection{Cooperation Tradeoff} 
\label{sec:cg-weight}
In this section, we explore the effects of varying degrees of cooperation on the performance of the resulting policy.

Fig.~\ref{fig:effect-of-cg-weights} depicts the effect of increasing cooperative penalties on the resulting policy in the \antgather environment. We define the degree of cooperation in comparison to the expected worker (or intrinsic) returns experienced in the standard hierarchical approach. The level of cooperation $l_\text{coop}$ is:
\begin{equation}
    l_\text{coop}(\delta) = \frac{Q_\text{w,HRL} - \delta}{Q_\text{w,HRL} - Q_\text{w,max}}
\end{equation}
where $Q_\text{w,HRL}$ is the (approximate) converged expected intrinsic returns by the standard HRL approach and $Q_\text{w,max}$ is the largest possible expected intrinsic returns.

In the \antgather task, we notice that expected intrinsic returns in the standard HRL approach converge to a value of about $-600$ (see Figure~\ref{fig:cg-delta-worker-qvals}). As a result, we promote cooperation by assigning values of $\delta$, or the desired expected intrinsic returns, that are progressively larger than $-600$ to determine what level of cooperation leads to the best performance. We define the degree of cooperation as the ratio of the $\delta$ constraint between the standard hierarchical approach and the maximum expected return (the intrinsic rewards used here are non-positive meaning that the largest expected return is $0$). For example, a $\delta$ value of $-450$ is equated to a level of cooperation $l_\text{coop}(-450) = (-600 + 450) / (-600 - 0) = 0.25$, or $25\%$.

% For $\lambda$ terms far beyond the optimal choice of $\lambda$ we see considerable reductions in performance: for small values of $\lambda$ the agent is incapable of making progress beyond standard HRL, while for large values of $\lambda$ that constraint on the higher-level policy is too severe to allow for training to progress. This finding then begs the question: What is an appropriate range for $\lambda$, and can this value be solved for during the training procedure?

Figures~\ref{fig:cg-delta-worker-qvals}~and~\ref{fig:cg-delta-lambda} depict the agent's ability to achieve the assigned $\delta$ constraint and the dynamic $\lambda$ terms assigned to achieve these constraints, respectively. For most choices of $\delta$, \methodName succeeds in defining dynamic $\lambda$ values that match the constraint. For very large constraints, in this case for $\delta=-50$, no choice of $\lambda$ can be assigned to match the desired constraint, thereby causing the value of $\lambda$ to grow exponentially.

% To answer these questions, we look to the constrained formulation of the cooperative HRL problem presented in Section~\ref{sec:method-constrained-hrl}. 

% Focusing once again on the \antgather environment, we notice that expected intrinsic returns in the standard HRL approach converges to a value of about $-600$ (see Figure~\ref{fig:cg-delta-worker-qvals}). We accordingly assign values for $\delta$, or the desired expected intrinsic returns, to values progressively larger than $-600$ in an attempt to determine what values
% % of $\lambda$ are required to achieve such constraints, and if these constraints 
% lead to improved performance by the policy as a whole.

Figures~\ref{fig:cg-delta-rewards}~to~\ref{fig:antgather-91.7p} depict the effect of varying levels of cooperation on the performance of the policy. As expected, we see that as the level of cooperation increases, the goal-assignment behaviors increasing consolidate near the path of the agent. This produces optimal behaviors in this setting for cooperation levels in the vicinity of 75\% (see Figures~\ref{fig:cg-delta-rewards}~and~\ref{fig:antgather-75p}). For levels of cooperation nearing 100\%, however, this consolidation begins to disincentivize forward movement, and subsequently exploration, by assignment goals that align with the current position of the agent (Figure~\ref{fig:antgather-91.7p}), thereby deteriorating the overall performance of the policy.
% These finding suggest that \st{blank}.

% \st{As we see in Figure}~\ref{fig:cg-delta-worker-qvals}\st{, our method is capable of assigning goals that maintain expected intrinsic returns greater than the desired estimate provided by $\delta$. We also find that constraining the goals such that the estimated worker returns are greater than $-150$ leads to improved behaviors over standard HRL. This constraint, as seen in Figure}~\ref{fig:cg-delta-lambda}\st{, updates the Lagrangian $\lambda$ term during training to values between $0.01$ and $0.025$. As we see in Figure}~\ref{fig:different-lambdas}\st{, the improvements seen by the policy within this environment is robust to fixed choices of $\lambda$ within this range. This suggests that constraining for estimates of the Worker Q-values improve the performance of standard hierarchical methods, and provides a range for appropriate values for $\lambda$. Further analysis is required to determine whether solving for fixed or dynamic $\lambda$'s are preferable in the context of hierarchical reinforcement learning.}

% When the value of $\lambda $ equals $0$, the algorithm is akin to the naive goal-conditioned HRL scheme as explained in Section~\ref{sec:no-cooperation}. For small values of $\lambda$, we witness improvements in intrinsic rewards that do not result in noticeable changes to the performance of the training algorithm. As we increase the $\lambda$ term, however, the increase in coordination begins to slow down improvements in environmental returns at the early stages of training. The corresponding increase in cooperation, however, results in a situation whereby the manager policy can confidently identify the effects of local goals on the actions the worker performs, ultimately allowing the overall policy to train much more efficiently. This initial slowing in training, however, begins to intensify for larger $\lambda$ terms in which the values of the worker gradient send too strong of a signal to the manager policy, thereby slowing down or stopping training completely. Interestingly enough, this does not result in significant improvement in the intrinsic returns from the most high-performing $\lambda$ term. These results suggest that moderate values of $\lambda$ are adequate to yield optimal results. 

% It is possible to construct a version of \methodName that has \textit{full} communication, meaning the optimization of the worker and manager is performed with a single loss. While this particular form of cooperation has worked well in MARL settings we found it performed poorly for HRL. We believe this is related to the frequency mismatch between the levels. The worker receives $k\times$ more data than the manager allowing it to have much better estimates of its Q function. 

% \subsection{Effects on non-stationarity}

% To increase the robustness of HRL methods that train multiple levels at the same time it would be beneficial to understand and limit the amount of \textit{non-stationarity} experienced by higher layers. Here we perform a version of the analysis from the view of the manager policy. We perform an examination of how much the worker policy distribution changes under the manager. The more this distribution changes the more variance that is introduced into the managers reward estimates. We find that the \methodName limits the amount of non-stationarity experienced by the manager and it appears to be a function of the $\lambda$ term. We show this comparison in~Fig.\ref{fig:ns} where we can see that \methodName achieves lower divergence and therefore lower non-stationarity issues. These reductions can be a partial indication as to why \methodName performs better than other methods compared to in this paper. In Appendix~\ref{sec:non-stationarity} we provide some mathematical motivation for why \methodName can reduce non-stationarity.


==> introduction.tex <==

\section{Introduction} \label{sec:introduction}

To solve interesting problems in the real world agents must be adept at planning and reasoning over long time horizons. For instance, in robot navigation and interaction tasks (Figures~\ref{fig:antgather-env}~to~\ref{fig:biped-sim}), agents must learn to compose lengthy sequences of actions to achieve long-term goals. In other environments, such as mixed-autonomy traffic control settings~\citep{wu2017emergent, vinitsky2018benchmarks} (Figures~\ref{fig:ring-env},~\ref{fig:highwaysingle-env}), exploration is delicate, as individual actions may not influence the flow of traffic until multiple timesteps in the future. RL has had limited success in solving long-horizon planning problems such as these without relying on task-specific reward shaping strategies that limit the performance of resulting policies~\citep{wu2017flow} or additional task decomposition techniques that are not transferable to different tasks~\citep{sutton1999between, kulkarni2016hierarchical, 2017-TOG-deepLoco, florensa2017stochastic}.

\begin{figure*}
\centering
\begin{subfigure}[b]{\textwidth}
\centering
\begin{tikzpicture}
    \newcommand \boxwidth {1.0}
    \newcommand \boxheight {\textwidth}
    \newcommand \boxoffset {0}

    % for y shift
    \draw (0, -0.15) node {};

    % \draw
    % (\boxoffset,              \boxoffset) -- 
    % (\boxheight + \boxoffset, \boxoffset) -- 
    % (\boxheight + \boxoffset, \boxwidth + \boxoffset) -- 
    % (\boxoffset,              \boxwidth + \boxoffset) -- 
    % (\boxoffset,              \boxoffset);

    \filldraw [limegreen] (0.455 * \textwidth,\boxwidth + \boxoffset - 0.5) circle (0.125);
    \draw [anchor=west]
    (0.47 * \textwidth, \boxwidth + \boxoffset - 0.5) node {\scriptsize Apple ($+1$)};

    \filldraw [red] (0.58 * \textwidth,\boxwidth + \boxoffset - 0.5) circle (0.125);
    \draw [anchor=west]
    (0.595 * \textwidth, \boxwidth + \boxoffset - 0.5) node {\scriptsize Bomb ($-1$)};

    \filldraw [blue] (0.705 * \textwidth, \boxwidth + \boxoffset - 0.5) circle (0.125);
    \draw [anchor=west]
    (0.72 * \textwidth, \boxwidth + \boxoffset - 0.5) node {\scriptsize High-level goal};

    \draw [dashed] 
    (0.840 * \textwidth, \boxwidth + \boxoffset - 0.5) -- 
    (0.875 * \textwidth, \boxwidth + \boxoffset - 0.5); 
    \draw [anchor=west]
    (0.88 * \textwidth, \boxwidth + \boxoffset - 0.5) node {\scriptsize Agent trajectory};
\end{tikzpicture}
\end{subfigure} \\ \vspace{-0.4cm}
\begin{tikzpicture}
    \draw[->] (0, 0) -- (0.06*\textwidth, 0);
    \draw[anchor=west] (0.065*\textwidth, 0) node {\scriptsize training iteration};

    \draw[->] (0.52*\textwidth, 0) -- (0.58*\textwidth, 0);
    \draw[anchor=west] (0.585*\textwidth, 0) node {\scriptsize training iteration};
    \draw (\textwidth, 0) {};
\end{tikzpicture}\\[-15pt]
\begin{subfigure}[b]{0.48\textwidth}
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/HRL/100000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/HRL/300000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/HRL/500000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/HRL/700000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/HRL/900000.pdf}
    \end{subfigure}
    \caption{Standard HRL}
    \label{fig:goaldists-standrd}
\end{subfigure}
\hfill
\begin{tikzpicture}
    \draw [dashed] (0,0) -- (0,2.5);
\end{tikzpicture}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/CHER/100000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/CHER/300000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/CHER/500000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/CHER/700000.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\linewidth]{figures/AntGather/CHER/900000.pdf}
    \end{subfigure}
    \caption{Cooperative HRL}
    \label{fig:goaldists-cooperative}
\end{subfigure}\\[-8pt]
\caption{Here the learned goal proposal distributions are shown for normal HRL and our method. Our agents develop more reasonable goal proposals that allow low-level policies to learn goal reaching skills quicker. The additional communication also allows the high level to better understand why proposed goals failed.}
\label{fig:goaldists}
\end{figure*}

%
% An example of this is the game Montezuma's Revenge, where classic techniques such as DQN fail to produce relevant temporally consistent behaviors from exploring short-term primitive actions~\cite{kulkarni2016hierarchical}. \todo{I can try to add a traffic example here too, but keeping it concise might be better.}
%%GB.11.03: This paragraph does not do a very good job of describing the problem. The reader needs to be lead down a interesting path of why this is an important problem. From this writing. The difficulty of the problem also needs to be expressed so the reader has an appreciation for the technical aspect of the paper and what the are solving.

Concurrent learning methods in hierarchical RL are promising approaches for automating the process of task decomposition to previously unexplored problems~\citep{levy2017hierarchical,nachum2018data,li2019sub}. 
% \st{These methods simplify learning in long term planning tasks by separating high-level reasoning from low-level skill acquisition into two simpler MDPs, thereby enabling learning across sequences of temporally extended skills as opposed to individual actions.}
%% Why are they more manageable? We want a nice flowing story that leads into why having a cooperate goal distribution will be an advantage.
% Most hierarchical methods require a large amount of engineering of the lower action primitives and only train a single layer at a time.
% This can severely limit the types of behaviors the agent can produce and as such the policy optimality.
% For hierarchical methods to be more optimal they need to train each level of the hierarchy concurrently. However, concurrently training multiple policies at the same time results in a difficult non-stationary optimization problem that can lead to poorer results.
The process of concurrently learning diverse skills and exploiting these skills to achieve a high-level objective, however, is a difficult task. In particular, at the early stages of training lower-level policies are unable to reach most goals assigned to them by a higher-level policy, and instead must learn to do so as training progresses.
% In this setting, the absence of explicit or directed feedback on the lower-level policy's ability to achieve certain goals 
% \textcolor{red}{As illustrated in Figure~TODO}, 
This exacerbates the credit assignment problem from the perspective of the higher-level policy, as it is unable to identify whether a specific goal under-performed as a result of the choice of goal or the lower-level policy's inability to achieve it. In practice, this results in the highly varying or random goal assignment strategies in~Figure~\ref{fig:goaldists-standrd} that require a large number of samples~\cite{li2019sub} and some degree of feature engineering~\cite{nachum2018data} to optimize over.
% and prevents the policy from performing intricate maneuvers that avoid undesirable states.

% More recently, the options and goal-conditioned formulations of hierarchical reinforcement learning (HRL) have become very popular. The options framework~\citep{sutton1999between} decomposes task execution to a sequence of \emph{options} capable of performing a diverse set of tasks (such as moving left, right, up, and down), and a \emph{policy over options} that chooses options that maximize the environmental return. This approach works very well when options can be defined apriori, but has experienced limited success in learning in a purely end-to-end fashion~\citep{bacon2017option}. In goal-conditioned~\citep{nachum2018data}, or feudal~\cite{dayan1993feudal, vezhnevets2017feudal}, HRL, on the other hand, higher-level manager policies assign goals in the form of desired states over extended period of times to a lower-level worker policy that then performs environmental actions that achieve these goals. This approach has been demonstrated to outperform the options framework in complex continuous control tasks, and is the hierarchical structure explored in this article.
%%GB.7.7: What does this last sentence add to the paragraph? Every sentence should provide clear and purposeful information in the paper. Or it should not be there. -- done
%%GB.7.7: This first paragraph is not clear enough. It is not articulating the problem well enough or in a general enough sense. I would suggest, talk about if we want intelligent agents they will need to solve long horizon tasks, starting with (i) it is important that agents solve these types of tasks (because most interesting tasks are long horizon, or we want to extend the horizon at which agents can be successful), then (ii) being able to solve these types of tasks gives the agents increased skill, which is important because..., (iii) This has been tricky for current flat methods. --TODO: second part

%%GB.7.7: Then a paragraph on why this problem is hard (some of the above paragraph can be reused here). (not easy to plan over long horizons, (ii) credit assignment issues, variance issues, data issues.
% Then discuss that one promising approach is to structure the problem in such a way to make reduce the planning horizon of the problem

% \todo{I removed the whole connection to MARL thing. We may want to reintroduce it, but I'm starting to get the sense that it results in more confusion than insight.}

In this paper, we pose this problem presented above as a result of insufficient cooperation between internal levels within a
hierarchy\footnote{The connection of this problem to cooperation in multiagent RL is discussed in Section~\ref{sec:algorithm}.}, and subsequently introduce mechanisms that promote variable degrees of cooperation in HRL.
Our approach improves cooperation by encouraging higher-level policies to specify goals that lower-level policies can succeed at,
thereby disambiguating under-performing goals from goals that were unachievable by the lower-level policy.
% 
% encourages cooperation between various levels of a hierarchy by redefining the objective of higher-level policies to directly account for losses experienced by lower-level policies,
%% To detailed and yet does not provide any information on what is really done.
% 
% The gradients associated with lower-level's capabilities are added to the loss of the higher-level policies are then propagated through its parameters by replacing the communication actions (or goals) by the higher-level policy during training with direct connections between its output and the input to the lower-level policy.
%% This sounds like to much detail and it breaking the flow again. Lets used the terms capability to describe what the low level can do.
% 
% In this paper,
% we improve the performance of goal-conditioned hierarchical reinforcement learning by introducing cooperation between policy levels. This cooperation influences the progression of learning and the agent's subsequent ability to perform complex tasks.
%% Want to make a connection to methods that create an automatic curriculum.
% we address these issues by 
% providing the capabilities of the lower-level to the higher-level and 
% introducing techniques that 
% encourage higher-level policies to specify goals the lower-level can succeed at.
% 
% 
In Figure~\ref{fig:goaldists}(b) we show how our method changes the high-level goal distributions to be within the capabilities of the agent. This approach results in more informative communication between the policies. 
%% The wording here could be improved more to claim a little more. What is the best conceptual way to describe the pros of the method.
Conceptually our method shares similarities to recent methods on automatic curriculum generation~\cite{wang2019paired, dennis2020emergent, held2017automatic} but between the evolution of two agents. The distribution of goals or tasks the high-level will command of the lower level expands over time as the lower-level policy's capabilities increase.
% \todo{GLEN: Include a bit more detail on how the method works. At least the conceptual sharing of values so that a person familiar with HRL will understand the idea.}

To promote cooperation in HRL, we take inspiration from
% Motivated by studies on 
differentiable communication~\citep{DBLP:journals/corr/SukhbaatarSF16,DBLP:journals/corr/FoersterAFW16a} and emergent cooperation phenomena~\citep{claus1998dynamics,panait2005cooperative} in multiagent RL.
% , we present a novel optimization procedure that addresses limitations in goal-assignment behaviors by promoting inter-level cooperation in HRL. 
Our approach attempts to encourage cooperation between various levels of a hierarchy by redefining the objective of higher-level policies to directly account for losses experienced by lower-level policies. The gradients of these additions to the loss are then propagated through the parameters of the higher-level policy by replacing the goals policy during training with direct connections to the lower-level policy.

% \textcolor{red}{Empirically, the loss-sharing paradigm presented in the article serves to promote cooperation by aligning goal-assignment strategies with achievable desired states by the goal-achieving worker policies. This serves to direct the exploration procedure within the vicinity of meaningful goals, thereby alleviating limitations brought about when searching through high-dimensional goal spaces. 
% This also helps reduce overestimation biases within the goal assignment procedure, which we find limits the performance of hierarchies for even low-dimensional tasks, such as assigning desired speeds to individual vehicles.
% In Section~\ref{sec:experiments}, we demonstrate the increased cooperation can expand the horizon of solvable tasks by HRL.}
% %% This paragraph sounds much better than the last to explain what is being done at a higher level.
% , a technique that was initial presented for multi-agent settings in~\cite{DBLP:journals/corr/FoersterAFW16a}.
%%GB.7.7: Again this should be saved for the related work section. Currently, we mention this paper many times and we can't describe why out method is new each time this paper is mentioned. This can lead to confusing the reader and in the worst case view our work as not very novel! We should move this to the related work section. -- TODO: move to related works
% Instead, in this work we expand this method and apply it a more restricted HRL communication problem that includes temporal abstraction in the communication. 
% The resultant gradient update procedure, which we call \emph{Cooperative HiErarchical RL} (\methodName), is empirically demonstrated to achieve superior performance on a variety of long-term horizon tasks, and further serves to expand the scope of solvable tasks by hierarchical reinforcement learning.
% \todo{And is more scalable? We need to sell this more.}
% This technique, which more closely resembles single agent policy optimization for hierarchical models, more readily promotes cooperation between levels of the policy, and as a result can significantly improve sample efficiency and training performance.
%%GB.11.03: The above paragraph sounds pretty good. However, it will be even better with a little more detail on how this communication is facilitated

% The key contributions of this paper are as follows:
% \begin{itemize}[leftmargin=1.5em]
%     % \item In order to solidify the connections between goal-conditioned hierarchical tasks and Markov games, we begin by formulating the HRL problem as a Markov game and demonstrate a potential limiting feature of existing policy update schemes in this setting.
%     % \nabla_{\theta_m} J_m' = \nabla_{\theta_m} \left( J_m + \lambda J_w \right) = \nabla_{\theta_m} J_m + \lambda \nabla_{\theta_m} J_w
%     \item We derive a new off-policy gradient algorithm for higher level policies in 
%     % a previously studied 
%     two-level hierarchical policies. Our technique, called \emph{Cooperative HiErarchical RL} (\methodName), is empirically demonstrated to achieve superior performance on a variety of long-term horizon tasks, and further serves to expand the scope of solvable tasks by hierarchical reinforcement learning.
%     \item Key to our technique is the ability to control the amount of cooperation between the HRL layers. As a result, we dedicate a portion of this paper on developing an intuition of the effects this particular cooperation mechanism can have on the evolution of the various levels.
% \end{itemize}
%%GB.11.03: These are very simple contributions. This should be turned into a paragraph and most importantly we need to discuss the new results that we are to achieve with some detail, not just say it worked and things are better. This is to vague. -- TODO

% \st{The introduced method controls the level of cooperation between the layers or modules of the HRL method. It allows the method to solve complicated navigation tasks as well as and better than previous work while scaling to higher dimensional states all due to a combination of reward functions. This combination allows the higher levels to prefer using goals that are high value for the lower level.}
%% It would be really great if we could get a 3 level hierarchy working on some example.

A key finding in this paper is that regulating the degree of cooperation between HRL layers can significantly impact the learned behavior by the policy. Too little cooperation may introduce no change to the goal-assignment behaviors and subsequent learning, while excessive cooperation may disincentivize an agent from making forward progress. We accordingly introduce a constrained optimization that serves to regulate the degree of cooperation between layers and ground the notion of cooperation in HRL to quantitative metrics within the lower-level policy. This approach results in a general and stable method for optimizing hierarchical policies together.

We demonstrate the performance of our method on a collection of standard HRL environments and two previously unexplored mixed autonomy traffic control tasks. For the former set of problems, we find that our method can achieve better performance compared to recent sample efficient off-policy and HRL algorithms.
For the mixed autonomy traffic tasks, the previous HRL methods struggle while our approach subverts overestimation biases that emerge in the early stages of training, thereby allowing the controlled (autonomous) vehicles to regulate their speeds around the optimal driving of the task as opposed to continuously attempting to drive as fast as possible.
%%GB.2.3: This paragraph still needs work. We need to describe the results of the method in as good a light as we can. However, we should not point to direct details of the algorithm here.

% This approach, as we expand upon in Section~\ref{sec:cg-weight}, allows us to explore the effects of varying degrees of cooperation on the performance of the policy.
%% This should discuss the dynamic cooperation formulation and how it works similar to a collection of papers that create automatic curriclum methods. This will help provide obvious reasoning about how this will provide an improvement.

% The remainder of the paper is organized as follows. Section~\ref{sec:background} provides background on MDPs, reinforcement learning, and HRL, and presents the hierarchical model utilized for the rest of the paper. Section~\ref{sec:method} introduces our approach to inducing cooperation in HRL and grounds the notion of cooperation in worker expected returns. Section~\ref{sec:related-work} finds connections with our work and others involving improved coordination with gradients, and draws similarities between insights from state-of-the-art HRL algorithms and methods for improving training performance in MARL domains. And finally, Section~\ref{sec:experiments} empirically compares our model with other hierarchical algorithms for various long horizon control and planning tasks ranging from agent navigation to mixed-autonomy traffic flow control.


==> method.tex <==
\section{Cooperative hierarchical reinforcement learning} \label{sec:method}

In this section, we introduce a technique for \emph{Cooperative HiErarchical RL}, which we call \methodName. \methodName promotes cooperation by propagating losses that arise from random or unachievable goal-assignment strategies. As part of this algorithm, we also present a mechanism to optimize the level of cooperation and ground the notion of cooperation in HRL to measurable variables. 
% The performance of this algorithm is explored in Section~\ref{sec:experiments}.

\subsection{Promoting cooperation via loss-sharing} \label{sec:algorithm}

\citet{tampuu2017multiagent} explored the effects of reward (or loss) sharing between agents on the emergence of cooperative and competitive in multiagent two-player games. Their study highlights two potential benefits of loss-sharing in multiagent systems: 1) emerged cooperative behaviors are less aggressive and more likely to emphasize improved interactions with neighboring agents, 2) these interactions reduce overestimation bias of the Q-function from the perspective of each agent.

% \st{where $\lambda$ is a weighting term that controls the level of cooperation the manager has with the worker. This term is in part motivated by studies on the dynamics and evolution of cooperative behaviors in MARL, and is to a certain extent similar to cooperative reward scheme $\rho$ in}~\cite{tampuu2017multiagent}\st{. As we present in Section}~\ref{sec:cg-weight}\st{, this term can have a significant effect of training performance.}
% We also note that a similar cooperative term is not supplied to the worker policy as it, by definition, is trained to cooperate with the goals issued to it by the manager.

% Given the similarities between HRL and MARL we explore methods that have been more successful in multi-agent learning to HRL, namely the assumption of cooperating agents. While we draw inspiration from multi-agent methods they can not be directly applied, due to the temporal abstraction between the layers in HRL.
% In response to this, we introduce a connected gradient formulation for training higher-level policies in two-level goal-conditioned hierarchies. The effects of this formulation on subsequent training is empirically studied in later sections.

% \st{In order to alleviate the training challenges described in the previous subsection, this paper redefines the higher-level objective function to directly promote cooperation by the manager policies with the policy directly below it.} 
In this article, we aim to explore the benefits of similar loss-sharing paradigms in goal-conditioned hierarchies. In particular, we focus on the emergence of collaborative behaviors from the perspective of goal-assignment and goal-achieving policies In line with prior work, we promote the emergence of cooperative behaviors by incorporating a weighted form of the worker expected return to the original manager objective $J_m$. Our new expected return is:
% To that end, we modify the expected return of the manager policy $J_m$ to include a weighted term for the worker expected return as well. Our new expected return, $J_m'$, is
\begin{equation} \label{eq:connected-return}
    J_m' = J_m + \lambda J_w
    % \begin{aligned}
    % &\resizebox{!}{7.5pt}{$
    %     J_m' = J_m + \lambda J_w 
    % $}\\
    % & \quad \ \ \resizebox{!}{12pt}{$
    %     = \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^{T/k} \left[ \gamma^t r_m(s_t) \right] \right]
    % $}\\
    % & \quad \quad \ \resizebox{!}{12pt}{$
    %     + \lambda \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^k \gamma^t r_w(s_t, g_t,\pi_w(s_t,g_t)) \right]
    % $}
    % \end{aligned}
\end{equation}
where $\lambda$ is a weighting term that controls the level of cooperation the manager has with the worker.

In practice, we find that this addition to the objective serves to promote cooperation by aligning goal-assignment actions by the manager with achievable trajectories by the goal-achieving worker. This serves as a regularizer to the manager policy: when presented with goals that perform similarly, the manager tends towards goals that more closely match the worker states. The degree to which the policy tends toward achievable states is dictated by the $\lambda$ term. The choice of this parameter accordingly can have a significant effect on learned goals. For large or infinite values of $\lambda$, for instance, this cooperative term can eliminate exploration by assigning goals that match the worker's current state and prevent forward movement (this is highlighted in Section~\ref{sec:cg-weight}). In Section~\ref{sec:method-constrained-hrl}, we provide intuitions for understanding the notion of cooperation in HRL by connecting it to measurable terms within the worker policy.

% The penalization of also prevents overestimation from taking place at the earlier stages of training by emphasizing penalizes goal assignment. How this relates to multiagent RL via communication and exploration.

\subsection{Cooperative gradients via differentiable communication}

To compute the gradient of the additional weighted expected return through the parameters of the manager policy, we take inspiration from similar studies in differentiable communication in MARL. The main insight that enables the derivation of such a gradient is the notion that goal states $g_t$ from the perspective of the worker policy are structurally similar to communication signals in multi-agent systems. As a result, the gradients of the expected intrinsic returns can be computed
% Under this new definition of the loss function, the worker loss is propagated 
% through the manager's trainable parameters 
by replacing the goal term within the reward function of the worker with the direct output from the manager's policy. This is depicted in Figure~\ref{fig:hrl-connected}. 

\begin{figure}
\centering
% \begin{minipage}[b]{0.95\textwidth}
% \begin{tikzpicture}
%     \newcommand \boxwidth {0.54}
%     \newcommand \boxoffset {0.36}
%     \newcommand \envwidth {5.76}
%     \newcommand \envheight {0.54}
%     \newcommand \layerwidth {1.44}
%     \newcommand \layerskip {1.008}

%     \draw[anchor=west] (-2, 5.7*\envheight/2) node {\small Standard};
%     \draw[anchor=west] (-2, 4.3*\envheight/2) node {\small HRL};

%     % environment box    
%     \fill [orange!30!white] (0,0) rectangle (\envwidth, \envheight);
%     \draw [brown] (0,0) -- (\envwidth,0);
%     \draw [brown] (0, \envheight) -- (\envwidth, \envheight);
%     \draw (\envwidth/2, \envheight/2) node {\small Environment};

%     % manager boxes
%     \filldraw [black!40!white, draw=black!90!white] 
%     (2*\boxoffset, 3.5*\envheight) rectangle 
%     (2*\boxoffset + \boxwidth, 3.5*\envheight + \boxwidth);
%     \draw
%     (2.0*\boxoffset + 0.5*\boxwidth, 3.5*\envheight + 0.5*\boxwidth) node {\scriptsize $\pi_m$};

%     % worker boxes
%     \filldraw [black!5!white, draw=black!15!white] 
%     (4.5*\boxoffset, 2*\envheight) rectangle 
%     (4.5*\boxoffset + \boxwidth, 2*\envheight + \boxwidth);

%     \filldraw [black!5!white, draw=black!15!white] 
%     (6.0*\boxoffset + 1.0*\boxwidth, 2*\envheight) rectangle 
%     (6.0*\boxoffset + 2.0*\boxwidth, 2*\envheight + \boxwidth);

%     \filldraw [black!20!white, draw=black!80!white] 
%     (9.0*\boxoffset + 2.0*\boxwidth, 2*\envheight) rectangle 
%     (9.0*\boxoffset + 3.0*\boxwidth, 2*\envheight + \boxwidth);
%     \draw
%     (9.0*\boxoffset + 2.5*\boxwidth, 2*\envheight + 0.5*\boxwidth) node {\scriptsize $\pi_w$};

%     % loss

%     \draw [red] [->] 
%     (5.5*\boxoffset + 0.5*\boxwidth, 3.75*\envheight) --
%     (3*\boxoffset + \boxwidth, 3.75*\envheight);
%     \draw 
%     (6*\boxoffset + \boxwidth, 3.75*\envheight) node {\small \color{red}{$\nabla \theta_m J_m$}}; 

%     \draw [red] [->] 
%     (10*\boxoffset + 3.0*\boxwidth, 1.75*\envheight) --
%     (10*\boxoffset + 3.0*\boxwidth, 3.25*\envheight) --
%     (8.5*\boxoffset + 3.0*\boxwidth, 3.25*\envheight);
%     \draw 
%     (13*\boxoffset + \boxwidth, 3.75*\envheight) node {\small \color{red}{$\nabla \theta_w J_w$}}; 

%     % connections

%     \draw [->] 
%     (1.25 * \boxoffset, \envheight) -- (1.25 * \boxoffset, 4 * \envheight) -- (2*\boxoffset, 4 * \envheight);
%     \draw [black!15!white] [->] 
%     (1.25 * \boxoffset, 2.5*\envheight) -- (4.5*\boxoffset, 2.5*\envheight);
%     \draw 
%     (1.25 * \boxoffset + 0.25, \envheight + 0.2) node {\small $s_t$}; 

%     \draw [->] 
%     (2*\boxoffset + \boxwidth, 4*\envheight) -- 
%     (4.5*\boxoffset + 0.5*\boxwidth, 4*\envheight);
%     \draw [black!15!white] [->] 
%     (4.5*\boxoffset + 0.5*\boxwidth, 4*\envheight) -- 
%     (4.5*\boxoffset + 0.5*\boxwidth, 3*\envheight);
%     \draw [black!15!white] [->] 
%     (4.5*\boxoffset + 0.5*\boxwidth, 4*\envheight) -- 
%     (4.5*\boxoffset + 2.5*\boxwidth, 4*\envheight) -- 
%     (4.5*\boxoffset + 2.5*\boxwidth, 3*\envheight);
%     \draw [black!15!white]
%     (4.5*\boxoffset + 2.5*\boxwidth, 4*\envheight) -- 
%     (5.5*\boxoffset + 2.5*\boxwidth, 4*\envheight); 
%     \draw 
%     (7.5*\boxoffset + 2.0*\boxwidth, 4.0*\envheight) node {\color{black!15!white}{$\cdots$}}; 
%     \draw [->]
%     (8.5*\boxoffset + 2.0*\boxwidth, 4*\envheight) -- 
%     (9.0*\boxoffset + 2.5*\boxwidth, 4*\envheight) --
%     (9.0*\boxoffset + 2.5*\boxwidth, 3*\envheight); 
%     \draw 
%     (2*\boxoffset + \boxwidth + 0.3, 4 * \envheight + 0.2) node {\small $g_t$}; 

%     \draw [black!15!white] [->] 
%     (4.5*\boxoffset + \boxwidth, 2.5*\envheight) --
%     (5.0*\boxoffset + \boxwidth, 2.5*\envheight) --
%     (5.0*\boxoffset + \boxwidth, 1.0*\envheight);
%     \draw
%     (5.0*\boxoffset + \boxwidth - 0.25, \envheight + 0.2) node {\small \color{black!15!white}{$a_t$}}; 

%     \draw [black!15!white] [->] 
%     (5.5*\boxoffset + \boxwidth, 1.0*\envheight) --
%     (5.5*\boxoffset + \boxwidth, 2.5*\envheight) --
%     (6.0*\boxoffset + \boxwidth, 2.5*\envheight);
%     \draw
%     (5.5*\boxoffset + \boxwidth + 0.4, \envheight + 0.2) node {\small \color{black!15!white}{$s_{t+1}$}}; 

%     \draw [black!15!white] [->] 
%     (6.0*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
%     (6.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
%     (6.5*\boxoffset + 2.0*\boxwidth, 1.0*\envheight);
%     \draw
%     (6.5*\boxoffset + 2.0*\boxwidth + 0.40, \envheight + 0.2) node {\small \color{black!15!white}{$a_{t+1}$}}; 

%     \draw (7.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) node {\color{black!15!white}{$\cdots$}}; 

%     \draw [->] 
%     (8.5*\boxoffset + 2.0*\boxwidth, 1.0*\envheight) --
%     (8.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
%     (9.0*\boxoffset + 2.0*\boxwidth, 2.5*\envheight);
%     \draw
%     (8.5*\boxoffset + 2.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $s_{t+i}$}; 

%     % cross out loss

%     \draw [red]
%     (8.5*\boxoffset + 2.0*\boxwidth - 0.2 - 0.1, 4*\envheight - 0.2) -- 
%     (8.5*\boxoffset + 2.0*\boxwidth + 0.2 - 0.1, 4*\envheight + 0.2); 
%     \draw [red]
%     (8.5*\boxoffset + 2.0*\boxwidth - 0.2 - 0.1, 4*\envheight + 0.2) -- 
%     (8.5*\boxoffset + 2.0*\boxwidth + 0.2 - 0.1, 4*\envheight - 0.2); 

%     \draw [->] 
%     (9.0*\boxoffset + 3.0*\boxwidth, 2.5*\envheight) --
%     (9.5*\boxoffset + 3.0*\boxwidth, 2.5*\envheight) --
%     (9.5*\boxoffset + 3.0*\boxwidth, 1.0*\envheight);
%     \draw
%     (9.5*\boxoffset + 3.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $a_{t+i}$};
% \end{tikzpicture}
% \end{minipage}%
% \\[5pt]
\centering
\begin{minipage}[b]{0.95\textwidth}
\begin{tikzpicture}
    \newcommand \boxwidth {0.65}
    \newcommand \boxoffset {0.5}
    \newcommand \envwidth {7.75}
    \newcommand \envheight {0.65}
    \newcommand \layerskip {1.4}

    % \draw[anchor=west] (-2, 5.7*\envheight/2) node 
    % {\small Cooperative};
    % \draw[anchor=west] (-2, 4.3*\envheight/2) node 
    % {\small HRL};

    % environment box    
    \fill [orange!30!white] (0,0) rectangle (\envwidth, \envheight);
    \draw [brown] (0,0) -- (\envwidth,0);
    \draw [brown] (0, \envheight) -- (\envwidth, \envheight);
    \draw (\envwidth/2, \envheight/2) node {\small Environment};

    % manager boxes
    \filldraw [black!40!white, draw=black!90!white] 
    (2*\boxoffset, 3.5*\envheight) rectangle 
    (2*\boxoffset + \boxwidth, 3.5*\envheight + \boxwidth);
    \draw 
    (2.0*\boxoffset + 0.5*\boxwidth, 3.5*\envheight + 0.5*\boxwidth) node {\scriptsize $\pi_m$};

    % worker boxes
    \filldraw [black!5!white, draw=black!15!white] 
    (4.5*\boxoffset, 2*\envheight) rectangle 
    (4.5*\boxoffset + \boxwidth, 2*\envheight + \boxwidth);

    \filldraw [black!5!white, draw=black!15!white] 
    (6.0*\boxoffset + 1.0*\boxwidth, 2*\envheight) rectangle 
    (6.0*\boxoffset + 2.0*\boxwidth, 2*\envheight + \boxwidth);

    \filldraw [black!20!white, draw=black!80!white] 
    (9.0*\boxoffset + 2.0*\boxwidth, 2*\envheight) rectangle 
    (9.0*\boxoffset + 3.0*\boxwidth, 2*\envheight + \boxwidth);
    \draw
    (9.0*\boxoffset + 2.5*\boxwidth, 2*\envheight + 0.5*\boxwidth) node {\scriptsize $\pi_w$};

    % loss

    \draw [red] [->] 
    (8.6*\boxoffset + 3.0*\boxwidth, 3.25*\envheight) --
    (8.6*\boxoffset + 3.0*\boxwidth, 4.00*\envheight);
    \draw 
    (13*\boxoffset + \boxwidth, 3.5*\envheight) node {\small \color{red}{$\nabla \theta_m J_w$}}; 

    % connections

    \draw [->] 
    (1.25 * \boxoffset, \envheight) -- (1.25 * \boxoffset, 4 * \envheight) -- (2*\boxoffset, 4 * \envheight);
    \draw [black!15!white] [->] 
    (1.25 * \boxoffset, 2.5*\envheight) -- (4.5*\boxoffset, 2.5*\envheight);
    \draw 
    (1.25 * \boxoffset + 0.25, \envheight + 0.2) node {\small $s_t$}; 

    \draw
    (2*\boxoffset + \boxwidth, 4*\envheight) -- 
    (5.5*\boxoffset + 2.5*\boxwidth, 4*\envheight); 
    \draw [black!15!white]
    (4.5*\boxoffset + 0.5*\boxwidth, 4*\envheight) -- 
    (4.5*\boxoffset + 0.5*\boxwidth, 3*\envheight);
    \draw [black!15!white]
    (4.5*\boxoffset + 2.5*\boxwidth, 4*\envheight) -- 
    (4.5*\boxoffset + 2.5*\boxwidth, 3*\envheight);
    \draw 
    (7.5*\boxoffset + 2.0*\boxwidth, 4.0*\envheight) node {$\cdots$}; 
    \draw [->]
    (8.5*\boxoffset + 2.0*\boxwidth, 4*\envheight) -- 
    (9.0*\boxoffset + 2.5*\boxwidth, 4*\envheight) --
    (9.0*\boxoffset + 2.5*\boxwidth, 3*\envheight); 
    \draw 
    (2*\boxoffset + \boxwidth + 0.3, 4 * \envheight + 0.2) node {\small $g_t$}; 

    \draw [black!15!white] [->] 
    (4.5*\boxoffset + \boxwidth, 2.5*\envheight) --
    (5.0*\boxoffset + \boxwidth, 2.5*\envheight) --
    (5.0*\boxoffset + \boxwidth, 1.0*\envheight);
    \draw
    (5.0*\boxoffset + \boxwidth - 0.25, \envheight + 0.2) node {\small \color{black!15!white}{$a_t$}}; 

    \draw [black!15!white] [->] 
    (5.5*\boxoffset + \boxwidth, 1.0*\envheight) --
    (5.5*\boxoffset + \boxwidth, 2.5*\envheight) --
    (6.0*\boxoffset + \boxwidth, 2.5*\envheight);
    \draw
    (5.5*\boxoffset + \boxwidth + 0.4, \envheight + 0.2) node {\small \color{black!15!white}{$s_{t+1}$}}; 

    \draw [black!15!white] [->] 
    (6.0*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
    (6.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
    (6.5*\boxoffset + 2.0*\boxwidth, 1.0*\envheight);
    \draw
    (6.5*\boxoffset + 2.0*\boxwidth + 0.40, \envheight + 0.2) node {\small \color{black!15!white}{$a_{t+1}$}}; 

    \draw (7.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) node {\color{black!15!white}{$\cdots$}}; 

    \draw [->] 
    (8.5*\boxoffset + 2.0*\boxwidth, 1.0*\envheight) --
    (8.5*\boxoffset + 2.0*\boxwidth, 2.5*\envheight) --
    (9.0*\boxoffset + 2.0*\boxwidth, 2.5*\envheight);
    \draw
    (8.5*\boxoffset + 2.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $s_{t+i}$}; 

    \draw [->] 
    (9.0*\boxoffset + 3.0*\boxwidth, 2.5*\envheight) --
    (9.5*\boxoffset + 3.0*\boxwidth, 2.5*\envheight) --
    (9.5*\boxoffset + 3.0*\boxwidth, 1.0*\envheight);
    \draw
    (9.5*\boxoffset + 3.0*\boxwidth + 0.40, \envheight + 0.2) node {\small $a_{t+i}$};
\end{tikzpicture}
\end{minipage}\\[-8pt]
\caption{An illustration of the 
% hierarchical 
policy gradient procedure. % \textbf{Top:} The actors for each level are trained to maximize separate rewards. No gradients are shared. 
% \textbf{Bottom:} 
To encourage cooperation, we introduce a 
% new 
gradient that propagates the rewards associated with the worker policies through the manager.
}
\label{fig:hrl-connected}
\end{figure}

The updated gradient is defined in Theorem~\ref{theorem} below.

\begin{theorem} \label{theorem}
Define the goal $g_t$ provided to the input of the worker policy $\pi_w(s_t,g_t)$ as the direct output from the manager policy $g_t$ whose transition function is:
\begin{equation}
    g_t(\theta_m) = 
    \begin{cases}
        \pi_m(s_t) & \text{if } t \text{ mod } k = 0 \\
        h(s_{t-1}, g_{t-1}(\theta_m), s_t) & \text{otherwise}
    \end{cases}
\end{equation}

where $h(\cdot)$ is a fixed goal transition function between meta-periods (see Appendix~\ref{sec:intrinsic-reward}). Under this assumption, the solution to the deterministic policy gradient~\cite{silver2014deterministic} of Eq.~\eqref{eq:connected-return} with respect to the manager's parameters $\theta_m$ is:
\begin{equation} \label{eq:connected-gradient}
    \resizebox{.9\hsize}{!}{$
    \begin{aligned}
        \nabla_{\theta_m} J_m' &= \mathbb{E}_{s\sim p_\pi} \big[ \nabla_a Q_m (s,a)|_{a=\pi_m(s)} \nabla_{\theta_m} \pi_m(s)\big] \\
        %
        &\quad + \lambda \mathbb{E}_{s\sim p_\pi} \bigg[ \nabla_{\theta_m} g_t \nabla_g \big(r_w(s_t,g,\pi_w(s_t,g_t)) \\
        & \quad + \pi_w (s_t,g) \nabla_a Q_w(s_t,g_t,a)|_{a=\pi_w(s_t,g_t)}\vphantom{\int} \big) \bigg\rvert_{g=g_t} \bigg]
    \end{aligned}
    $}
\end{equation}
where $Q_m(s,a)$ and $Q_w(s,g,a)$ are approximations for the expected environmental and intrinsic returns, respectively.
\end{theorem}

\vspace{-6pt}

\textit{Proof.} See Appendix~\ref{sec:derivation}.

This new gradient consists of three terms. The first and third term computes the gradient of the critic policies $Q_m$ and $Q_w$ for the parameters $\theta_m$, respectively. The second term computes the gradient of the worker-specific reward for the parameters $\theta_m$. This reward is a design feature within the goal-conditioned RL formulation, however, any reward function for which the gradient can be explicitly computed can be used. We describe a practical algorithm for training a cooperative two-level hierarchy implementing this loss function in Algorithm~\ref{alg:training}.

\subsection{Cooperative HRL as constrained optimization}
\label{sec:method-constrained-hrl}

In the previous sections, we introduced a framework for inducing and studying the effects of cooperation between internal agents within a hierarchy. The degree of cooperation is defined through a hyperparameter ($\lambda$), 
% \todo{Content was removed from here to help the story flow more smoothly.}
and if properly defined can greatly improve training performance in certain environments. The choice of $\lambda$, however,
% which 
can be difficult to specify without a priori knowledge of the task it is assigned to.
% \footnote{Potential factors that affect this of $\lambda$ choice include the relative scale of the rewards assigned to the higher and lower-level policies.}. 
We accordingly wish to ground the choice of $\lambda$ to measurable terms that can be reasoned and adjusted for. To that end, we observe that the cooperative $\lambda$ term acts equivalently as a Lagrangian term in constrained optimization~\citep{bertsekas2014constrained} with the expected return for the lower-level policy serving as the constraint. 
Our formulation of the HRL problem can similarly be framed as a constrained optimization problem, denoted as:
\begin{equation}
    \resizebox{.9\hsize}{!}{$
    \begin{aligned}
        &\max_{\pi_m} \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^{T/k} \left[ \gamma^t r_m(s_t) \right] \right] \\
        &\quad + \min_{\lambda\geq 0} \left( \lambda \delta - \lambda \min_{\pi_w} \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^k \gamma^t r_w(s_t, g_t,\pi_w(s_t,g_t)) \right] \right)
    \end{aligned}
    $}
\end{equation}
where $\delta$ is the desired expected discounted \emph{intrinsic} returns. The derivation of this equation and practical implementations are provided in Appendix~\ref{sec:constrained-hrl}.

\begin{figure*}
\centering
\begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[height=2.45cm]{figures/ring-env.png}
    \caption{\label{fig:ring-env} \footnotesize \ringroad}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.72\textwidth}
    \centering
    \includegraphics[height=2.45cm]{figures/highway-single-env.png}
    \caption{\footnotesize \highwaysingle}
    \label{fig:highwaysingle-env}
\end{subfigure} \\ \vspace{0.4cm}
\begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=2.75cm]{figures/AntGather-env.png}
    \caption{\label{fig:antgather-env} \footnotesize \antgather}
\end{subfigure}
\
\begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=2.75cm]{figures/AntFourRooms-env.png}
    \caption{\label{fig:antfourrooms-env} \footnotesize \antfourrooms}
\end{subfigure}
\
\begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[height=2.75cm]{figures/AntMaze-env.png}
    \caption{\label{fig:antmaze-sim} \footnotesize \antmaze}
\end{subfigure}
\
\begin{subfigure}[b]{0.34\textwidth}
    \centering
    \includegraphics[height=2.75cm]{figures/soccer_env.png}
    \caption{\label{fig:biped-sim} \footnotesize \bipedalsoccer}
\end{subfigure}\\[-8pt]
\caption{
Training environments explored within this paper. We compare the performance of various HRL algorithms on two mixed-autonomy traffic control task (a,b), three ant navigation tasks (c,d,e), and a bipedal/humanoid navigation task (d). A description of each of these environments is provided in Section~\ref{sec:environments}.
}
\label{fig:envs}
\end{figure*}

% For deterministic actor-critic methods such as DDPG~\citep{lillicrap2015continuous}, we can approximate the discounted \emph{intrinsic} returns through the worker's Q-function $Q_w$. The constrained formulation can accordingly be rewritten as:
% \begin{equation}
%     \resizebox{!}{26pt}{$
%     \begin{aligned}
%     &\max_{\pi_m} \mathbb{E}_{s\sim p_\pi} \left[ \sum_{t=0}^{T/k} \left[ \gamma^t r_m(s_t) \right] \right] \\
%     & \quad + \min_{\lambda\geq 0} \left( \lambda \delta - \lambda Q_w(s_t, g_t,\pi_w(s_t,g_t)) \right)
%     \end{aligned}
%     $}
% \end{equation}
In practice, this updated form of the objective provides two meaningful benefits: 1) As discussed in Section~\ref{sec:cg-weight}, it introduces bounds for appropriate values of $\delta$ that can then be explored and tuned, and 2) for the more complex and previously unsolvable tasks, we find that this approach results in more stable learning and better performing policies.

% Following this formulation, the choice of $\lambda$ is not fixed apriori, but can rather be solved for via dual gradient descent to match the desired behavior dictated by a newly defined $\delta$ term (this is expanded upon in Appendix~\ref{sec:constrained-hrl}). The choice of $\delta$ as a constraint can also simply be defined to promote varying degrees of cooperation through feedback from measurable estimates, in this case the worker Q-function. In Section~\ref{sec:cg-weight}, we provide simple intuitions for assigning the choice of $\delta$ and demonstrate the effect of this choice of $\delta$ on resulting behaviors.


==> related_work.tex <==
\section{Related Work} \label{sec:related-work}

%%GB.11.03: With the way the current paper is written I would move this earlier to help promote that this work is novel and that HRL is a very promising direction, we just need to work out a few last issues to make it more robust and accessible.

% Recent work has proposed a hierarchical policy gradient that promotes the use of a combined manager/worker loss~\cite{li2019sub}. Our work differentiates from this work primarily in three respects. First off, our derivation of the gradient applies to actor-critic algorithms, which have been empirically demonstrated to be significantly more data-efficient~\cite{fujimoto2018addressing, haarnoja2018soft}, and, being off-policy algorithms, may suffer even more greatly from the non-stationary effects associated with poor cooperation~\cite{nachum2018data}. Moreover, their implementation does not propose the use of weighting term $\lambda$ when combining the two gradients. This term, as we detail in Section~\ref{sec:cg-weight}, can have a significant effect of improving training performance. Finally, we take the gradient of the return of the manager with respect to the  worker in order to use connected gradients to propagate information up from the worker to the manager, whereas their purpose is to calculate the gradient of the trajectory with respect to both manager and worker. 

The topic explored in this article takes inspiration in part from studies of communication in multiagent reinforcement learning (MARL)~\citep{thomas2011conjugate, thomas2011policy, DBLP:journals/corr/SukhbaatarSF16, DBLP:journals/corr/FoersterAFW16a}. 
% 
In MARL, communication channels are often shared among agents as a means of coordinating and influencing neighboring agents.
%%GB.11.03: This part so far sounds very much like related work. This paragraph should instead be about a high level idea on how the method can be solved and how it will address the overarching ideas in the abstract (training multi-level policies because they are very promising in solving difficult tasks). -- TODO: move to related works section
% often refers to actions performed by individual agents in addition to their typical environmental action. These communication channels are perceived by the other agents and accordingly help coordinate and influence neighboring agents. 
Challenges emerge, however, as a result of the ambiguity of communication signals in the early staging of training, with agents forced to coordinate between sending and interpreting messages~\citep{mordatch2018emergence, eccles2019biases}. Similar communication channels are present in the HRL domain, with higher-level policies communicating one-sided signals in the form of goals to lower-level policies. The difficulties associated with cooperation, accordingly, likely (and as we find here in fact do) persist under this setting. The work presented here serves to make connections between these two fields, and will hopefully motivate future work on unifying the challenges experienced in each.

Our work is most motivated by the Differentiable Inter-Agent Learning (DIAL) method proposed by~\citet{DBLP:journals/corr/FoersterAFW16a}. Our work does not aim to learn an explicit communication channel; however, it is motivated by a similar principle - that letting gradients flow across agents results in richer feedback. Furthermore, we differ in the fact that we structure the problem as a hierarchical reinforcement learning problem in which agents are designed to solve dissimilar tasks. This disparity forces a more constrained and directed objective in which varying degrees of cooperation can be defined. This insight, we find, is important for ensuring that shared gradients can provide meaningful benefits to the hierarchical paradigm.
%%GB.2.3: This still does not say how CHER is better in this case. That needs to be pointed out. 

Another prominent challenge in MARL is the notion of \emph{non-stationarity}~\citep{busoniu2006multi, weinberg2004best, foerster2017stabilising}, whereby the continually changing nature of decision-making policies serve to destabilize training.
% \footnote{The notion of non-stationarity in HRL and its connection to MARL is expanded upon in Appendix~\ref{sec:non-stationarity}.}. 
This has been identified in previous studies on HRL, with techniques such as off-policy sample relabeling~\citep{nachum2018data} and hindsight~\citep{levy2017hierarchical} providing considerable improvements to training performance. Similarly, the method presented in this article focuses on non-stationary in HRL, with the manager constraining its search within the region of achievable goals by the worker. Unlike these methods, however, our approach additionally accounts for ambiguities in the credit assignment problem from the perspective of the manager. As we demonstrate in Section~\ref{sec:experiments}, this cooperation improves learning across a collection of complex and partially observable tasks with a high degree of stochasticity. These results suggest that multifaceted approaches to hierarchical learning, like the one proposed in this paper, that account for features such as information-sharing and cooperation in addition to non-stationarity are necessary for stable and generalizable HRL algorithms.
% These findings suggest that concepts of cooperation and information sharing between levels of hierarchy can play a pivotal role in producing generalizable and scalable hierarchical control algorithms.
% \todo{G: This ending still needs more work. The reader needs to see the obvious difference to prior work and clear benefit.}
%%GB.2.3: Here I am worried CHER does not sound very interesting.
% These studies, while not explicitly identifying the multi-agent nature training as a source of training instabilities, validate the notion that bottlenecks experienced in multi-agent training are in fact present in hierarchical reinforcement learning as well. \st{TODO: mention compositionality, that unlike these we can transfer our insights to on-policy methods as well.}

% \st{While hierarchical policies improve exploration and reduce the effective learning horizon of a given task, such models also decompose the policy into a set of independent actors that solve disparate optimization problems. This renders hierarchical policy optimization similar to \emph{multi-agent reinforcement learning} (MARL)}~\cite{hu2003nash, srinivasan2010innovations}\st{, which results in training challenges of its own}~\cite{matignon2012independent,hernandez2019survey,nguyen2020deep}\st{, notably non-stationarity}~\cite{busoniu2006multi, weinberg2004best, foerster2017stabilising}\st{ and mixed cooperative and competitive behaviors}~\cite{tampuu2017multiagent, claus1998dynamics, tan1993multi}. 
%%GB.7.21: This is still an issue.
% In recent years, some of these challenges, most notably non-stationarity, have been identified as limiting features in HRL as well~\cite{nachum2018data,levy2017hierarchical}, thereby validating the notion that bottlenecks experienced in multi-agent training are in fact present in hierarchical reinforcement learning as well, and serving to further motivate the analysis hierarchical models in RL from the perspective of multi-agent systems.
%
% \st{While previous studies have accounted for non-stationarity in HRL}~\cite{nachum2018data, levy2017hierarchical}\st{, this paper focuses on a separate connection between hierarchical and multi-agent RL, namely the concept of utilizing communication for facilitating intra-agent cooperation}~\cite{hausknecht2016cooperation,hernandez2019survey}.

% Finally, goal-conditioned hierarchical reinforcement learning has been a useful paradigm in increasing cooperation between multiple levels of a hierarchy~\cite{vezhnevets2017feudal, levy2017hierarchical,frans2017meta}; a proposed improvement has been using representation learning through a goal embedding. This idea has been proposed in \cite{DBLP:journals/corr/abs-1810-01257} and can be seen as an extended form of communication, wherein they try to convey the most relevant information in a compressed format to induce greater cooperation.

% \todoGlen{We should include a paragraph on goal conditioned RL and hierarchical RL. Then intrinsic reward methods. The similar MARL methods.}

